Efficient Map Prediction via Low-Rank Matrix Completion

In many autonomous mapping tasks, the maps cannot be accurately constructed due to various reasons such as sparse, noisy, and partial sensor measurements. We propose a novel map prediction method built upon the recent success of Low-Rank Matrix Completion. The proposed map prediction is able to achieve both map interpolation and extrapolation on raw poor-quality maps with missing or noisy observations. We validate with extensive simulated experiments that the approach can achieve real-time computation for large maps, and the performance is superior to the state-of-the-art map prediction approach - Bayesian Hilbert Mapping in terms of mapping accuracy and computation time. Then we demonstrate that with the proposed real-time map prediction framework, the coverage convergence rate (per action step) for a set of representative coverage planning methods commonly used for environmental modeling and monitoring tasks can be significantly improved.

==> icra21-final/0_abstract.tex <==
\begin{abstract}
In many autonomous mapping tasks, the maps cannot be accurately constructed due to various reasons such as sparse, noisy, and partial sensor measurements.  
We propose a novel map prediction method built upon recent success of \textit{Low-Rank Matrix Completion}. The proposed map prediction is able to achieve both map interpolation and extrapolation on raw poor-quality maps with missing or noisy observations. 
We validate with extensive simulated experiments that the approach can achieve real-time computation for large maps, and the performance is superior to state-of-the-art map prediction approach --- Bayesian Hilbert Mapping in terms of mapping accuracy and computation time.
Then we demonstrate that with the proposed real-time map prediction framework, the coverage convergence rate~(per action step) for a set of representative coverage planning methods commonly used for environmental modeling and monitoring tasks can be significantly improved.

\end{abstract}

==> icra21-final/1_introduction.tex <==
\section{INTRODUCTION}
Mapping is a critical functionality for an autonomous robot that needs to perform tasks in an initially unknown environment where an underlying map is constructed with onboard sensors. 
However, this can be challenging if the sensor measurements are inaccurate or if the environment can only be partially measured (sensed), which are commonly seen in autonomous mapping scenarios. 
For instance, the point clouds obtained from low-end proximity sensors (e.g., LiDAR, IR, Sonar) might be extremely sparse especially in spacious environments. The point clouds might also contain many outliers (noisy points). In addition, oftentimes a mapping robot cannot visit every spot of the environment and the traversed areas may only partially cover the space with only some small sub-regions being measured. 
Given the sparse, noisy, and partial observations, it is desirable that a complete map can be efficiently predicted to well match the ground-truth environment, which is the objective of this paper. 

More formally, the map prediction aims to predict map structure based on already known regions and could be categorized into two classes: interpolation and extrapolation. Map interpolation means given some observations (measurement samples), we want to predict the values \textit{in between} the sampled places;
Map extrapolation means given some observation samples (or map structures), we want to predict the map values \textit{beyond} the sampled places. 

\begin{figure} \vspace{5pt}
  \centering
%   \subfigure[]
  	{\label{fig:real}\includegraphics[width=\linewidth]{figs/real_examples.png}}
  \caption{\small Urban and residential environments reveal strong structured patterns, such as \textit{Left}: road (or street) network and \textit{Right}: buildings layout. These environments containing linear dependent structures can be modeled as low-rank-matrix maps.} 
\label{fig:real}  
\end{figure}


In this paper, we propose to use Low-Rank Matrix Completion~(LRMC) to leverage the ill-conditioned map data to predict the whole map. LRMC exploits some special structures, such as low rank~(or linear dependency) and incoherence hidden in underlying map to perform the prediction. Two examples that possess special patterns in urban/residential environments are shown in Fig.~\ref{fig:real}.
We first illustrate how a structured environmental map satisfies important assumptions required by LRMC model. Then we qualitatively demonstrate with an urban road network map that our proposed LRMC method outperforms state-of-the-art map prediction~(or regression) method -- Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian} which is a Bayesian extension of Hilbert Mapping~(HM)~\cite{ramos2016hilbert}, where the map prediction is treated as a kernelized logistic regression problem. BHM eliminates crucial regularization parameter tunning in HM, and outputs continuous maps where the occupancy value of any arbitrary point could be queried.

We conduct exhaustive simulations on a set of maze-like complex maps and quantitatively analyze that our proposed LRMC method is superior to BHM on the maps with varying linear patterns and different rank values. 
Finally we combine the proposed real-time map prediction with representative coverage planning methods commonly used for environmental mapping and monitoring, and show that the mapping coverage convergence could be significantly improved with high mapping accuracy. 

We summarize our contributions as follows:
\begin{itemize}
    \item 
    This is the first time to examine and report that many complex urban/residential environments possess low-rank and incoherent structure, and to apply Low-Rank Matrix Completion for map prediction based on sparse, noisy, and partially observed maps.
    \item
    Our proposed Low-Rank Matrix Completion based map prediction outperforms state-of-the-art map prediction method---Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and is able to perform prediction in real-time.
    \item
    We perform extensive simulations and demonstrate the remarkable effectiveness of our proposed method  which allows representative coverage planning methods to achieve faster mapping coverage convergence rates.  %commonly used in environmental mapping   can be substantially improved.
\end{itemize}


==> icra21-final/2_related_work.tex <==
\section{RELATED WORK}

Map prediction has been studied in occupancy mapping problems.  
Prevalent methods include Occupancy Girds Mapping~(OGM)~\cite{elfes1989using}, Gaussian Process Occupancy Mapping~(GPOM)~\cite{o2012gaussian, wang2016fast}, Hilbert Mapping~(HM)~\cite{ramos2016hilbert} and Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian}. Specifically, OGM belongs to discrete mapping and all grids are independent with each other. To eliminate the requirement of pre-defining discrete grids and the independence assumption in OGM, GPOM is proposed and used in many applications~\cite{jadidi2014exploration, jadidi2015mutual}. GPOM naturally captures the neighbouring information thanks to kernelization, but being a non-parametric model, it has a computation complexity of $O(n^3)$, where $n$ is the number of sampled data points. Combining various advantages of GPOM, a faster and simpler parametric model---HM and its Bayesian version, BHM, is proposed later to eliminate the cubical time complexity in GPOM.

Map extrapolation 
attracts increasing attention in recent years and almost all the current methods for map extrapolation are based on deep neural networks~(DNNs)~\cite{caley2019deep, pronobis2017learning, katyal2018occupancy, shrestha2019learned, saroya2020online, katyal2019uncertainty}. However, DNNs based methods require huge amount of data for training and hence are still limited in general applications. In this paper, we propose to use Low-Rank Matrix Completion to perform the map prediction. 
Our proposed LRMC based method falls in between the {interpolation} and {extrapolation} methods. Specifically, the LRMC method can not only well interpolate map values, but at the same time can  extrapolate the map structure beyond the explored areas. 

In the past two decades, the Low-Rank Matrix Completion~(LRMC) problem has been well studied. The first theoretically guaranteed exact LRMC algorithm is proposed in~\cite{candes2009exact}, where any $n \times n$ incoherent matrices of rank $r$ are proven to be exactly recovered from $C n^{1.2}r\log n$ uniformly randomly sampled entries with high probability through solving a convex problem of nuclear norm minimization~(NNM). Subsequent works~\cite{candes2010power, chen2015incoherence, gross2011recovering, recht2011simpler} refine the provable completion results following the NNM based method. However, since all of the algorithms mentioned above are based on second order methods~\cite{liu2010interior}, they can become extremely expensive if the matrix dimension is large~\cite{cai2010singular}. Some first order based methods~\cite{cai2010singular, ji2009accelerated, mazumder2010spectral} are developed later. They solve the nuclear norm minimization problem in an iterative manner and rely on Singular Value Decomposition~(SVD) of matrices and are suited to large-scale matrix completion problems. In recent years, many other techniques are developed, such as coherent matrix completion~\cite{liu2017new, bhojanapalli2014universal, chen2014coherent}, non-linear matrix completion~\cite{eriksson2012high} and adaptive sampling~\cite{chen2015completing, eftekhari2018mc2}. {\color{black}A recent survey on LRMC could be found in \cite{nguyen2019low}.}
In this paper, we mainly employ the first order SVD based iterative method, such as~\cite{mazumder2010spectral} to solve the LRMC problem. {\color{black} The SVD based methods are able to achieve low prediction error and maintain a low time complexity if certain special problem structure is appropriately leveraged~\cite{mazumder2010spectral}.}


==> icra21-final/3_methodology.tex <==
\section{METHODOLOGY}
\label{sect:method}

\subsection{Problem Description}
Map prediction exhibits the same form as the matrix completion \cite{recht2009simpler} while a 2D map can be treated as a matrix. We propose to use LRMC as the map prediction method. LRMC is defined as completing a partially observed matrix $\tilde{\mathbf{M}}\in\mathbb{R}^{n_1\times n_2}$ whose part of entries are missing and the corresponding ground-truth matrix $\mathbf{M}$ has a low-rank and incoherent structures. Since the ground-truth rank is usually unknown, a typical way to complete $\tilde{\mathbf{M}}$ is to find a minimal rank matrix $\mathbf{X}^*$ that is consistent with $\tilde{\mathbf{M}}$ on the observed entries. A formal mathematical definition is:
\begin{equation}
    \label{eq:mc_1}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&rank(\mathbf{X})\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega,
    \end{aligned}
\end{equation}
where $\Omega \subset \left \{ 1, \cdots, n_1 \right \}\times \left \{ 1, \dots, n_2 \right \} $ is an index set of locations corresponding to the observed entries~($\left ( i, j \right )\in \Omega$ if $M_{ij}$ is observed). 

\subsection{Low-Rank and Incoherent Structures}
Two important assumptions for the underlying matrix $\mathbf{M}$ must be satisfied to guarantee the matrix completion results:
\begin{itemize}
    \item 
    $\mathbf{M}$ should be a low-rank matrix. A low-rank matrix implies its rank value is much smaller than its dimension and this structure enables the possibility to leverage linear dependencies among columns and/or rows of a matrix to predict missing entries~\cite{ongie2018tensor}. 
    \item
    $\mathbf{M}$ should be an incoherent matrix, which means the coherence of $\mathbf{M}$ is low. Suppose that a \textit{compact} SVD of a rank-r matrix $\mathbf{M}\in \mathbb{R}^{n_1\times n_2}$ is $\mathbf{M} = \mathbf{U}\Sigma\mathbf{V}^T$, where $\mathbf{U} \in \mathbb{R}^{n_1\times r}$ and $\mathbf{V}\in \mathbb{R}^{n_2\times r}$ are stacked left and right singular vectors of $\mathbf{M}$, while $\Sigma \in \mathbb{R}^{r\times r}$ is the diagonal matrix formed by a number of $r$ singular values of $\mathbf{M}$. The statistical leverage scores of $\mathbf{U}$ and $\mathbf{V}$ are defined by $\gamma_{U} = \underset{i\in \left \{ 1, \cdots, n_1 \right \}}{\text{max}}\left \| \mathbf{U}_{i,~:} \right \|^2_2$ and $\gamma_{V} = \underset{j\in \left \{ 1, \cdots, n_2 \right \}}{\text{max}}\left \| \mathbf{V}_{j,~ :} \right \|^2_2$, respectively, where $\mathbf{U}_{i,~:}$ and $\mathbf{V}_{j,~:}$ represent the $i^{th}$ and $j^{th}$ row of $\mathbf{U}$ and $\mathbf{V}$. Then the coherence of $\mathbf{M}$ is defined as:
    \begin{equation}
        \label{eq:coherence}
        \gamma_{M} = \max \left \{ \gamma_{U}, \gamma_{V} \right \}.
    \end{equation}
    The value of $\gamma_M$ is within $\left [ 0, 1 \right ]$ and an incoherent structure means the value of $\gamma_M$ is near 0. A small coherence value implies that the mass of values in the matrix will not concentrate on small portions, but spread out through the whole matrix.
\end{itemize}

Under the two conditions, the matrix $\tilde{\mathbf{M}}$ has been shown to be provably recoverable~\cite{candes2009exact}. Fig.~\ref{fig:mazes_1} and Table~\ref{tb:maze_prop} illustrate the trends of ranks and coherences of different structured environments which are similar to complex versions of either urban road networks or building layouts.
We can observe that the typical structured environments have ranks below 100, which are significantly smaller compared to the original matrix dimensions which could be multiple magnitudes higher (e.g., $10^4$ or above). 
The trend of ranks also reflects the complexity of the environment, and the higher the rank is, the more complex the environment is.
Along with the rank values, we also list the coherence values computed by using Eq.~(\ref{eq:coherence}).
Although the coherence increases proportionally to the rank, they all stay at a low level indicating high incoherence. 

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:mazes_1}\includegraphics[width=0.99\linewidth]{figs/mazes_with_ranks.png}}
  \caption{\small Maze environments with different ranks.
  } \vspace{-10pt}
\label{fig:mazes_1}  
\end{figure}

\begin{table}[h]

\caption{Matrix properties of maze environments} %title of the table
\centering % centering table
\begin{tabularx}{\linewidth}{ccccccc}%{c rrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & (a) & (b) & (c) & (d) & (e) & (f)\\
\hline % inserts single-line
Rank & 2 & 7 & 11 & 14 & 19 & 22\\ % Entering row contents
Coherence & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabularx}
\label{tb:maze_prop}
\end{table}


\subsection{Solving LRMC in Map Prediction}
\label{sect:static}

To solve the LRMC problem, 
the rank minimization problem in Eq.~(\ref{eq:mc_1}) is non-convex and NP-hard unfortunately, and hence of little practical use. An alternative way for Eq.~(\ref{eq:mc_1}) is to replace $rank(\mathbf{X})$ with $\left \| \mathbf{X} \right \|_*$, where $\left \| \mathbf{X} \right \|_*$ is the nuclear norm of $\mathbf{X}$, that is, the sum of sigular values of $\mathbf{X}$: $\left \| \mathbf{X} \right \|_* = \sum_{k=1}^{\min \left \{ n_1, n_2 \right \}}\sigma_k(\mathbf{X})$, where $\sigma_k(\mathbf{X})$ is the $k^{th}$ largest singular values of $\mathbf{X}$. The new formulation is:
\begin{equation}
    \label{eq:mc_2}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega.
    \end{aligned}
\end{equation}
The nuclear norm $\left \| \mathbf{X} \right \|_*$ is an effective convex relaxation to the rank objective and the optimization in Eq.~(\ref{eq:mc_2}) could be solved by semi-definite programming~\cite{laurent2014positive}.

Nevertheless, the optimizations in Eq.~(\ref{eq:mc_1}) and Eq.~(\ref{eq:mc_2}) aim to exactly recover the partially observed matrix, and this way was claimed as too rigid and may result in over-fitting~\cite{mazumder2010spectral}. A more robust way is to add a regularization parameter in Eq.~(\ref{eq:mc_2}):
\begin{equation}
    \label{eq:mc_3}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && \sum_{(i, j)\in \Omega}(X_{ij} - M_{ij})^2\leq \delta,
    \end{aligned}
\end{equation}
where $\delta \geq 0$ is a parameter regulating the training error tolerance. Equivalently Eq.~(\ref{eq:mc_3}) could be reformulated in a Lagrange form:
\begin{equation}
    \label{eq:mc_4}
    \begin{aligned}
        \mathbf{X}^* = \underset{\mathbf{X}}{\text{argmin}} \sum_{(i, j)\in \Omega} (X_{ij} - M_{ij})^2 + \lambda \left \|\mathbf{X} \right \|_{*},
    \end{aligned}
\end{equation}
where $\lambda$ is a regularization parameter controlling the nuclear norm. A SVD based iterative method proposed in~\cite{mazumder2010spectral} can be used to solve the Eq.~(\ref{eq:mc_4}).


\subsection{Mapping with Non-myopic Planner}
\label{sect:plan}

We are intrigued if the proposed map prediction can facilitate and improve existing environmental mapping and coverage methods. Popular planning paradigms include lawnmower mapping~\cite{li2019coverage, song2018varepsilon}, myopic (short-horizon) planning~\cite{khan2014greedy}, as well as non-myopic (long-horizon) planning~\cite{ kantaros2019asymptotically}. Lawnmower planning pursues complete spatial coverage, and myopic methods are oftentimes greedy schemes. The non-myopic approaches have been favored by many researchers for environmental mapping and monitoring~\cite{ma2016information, chen2019pareto}. Since non-myopic planners optimize paths over some horizon, we adopt and adapt the standard  \textit{Traveling Salesman Problem}~(TSP), which will be used in our evaluation in the experimental section. 

A TSP 
can be defined as that, given the positions of a collection of way points, what is the shortest possible path of reaching each way point only once and eventually returning to the starting point. 
To efficiently solve the TSP, we extend our recently developed adaptive \textit{k}-opt method~\cite{ma2016adaptive} which exploits and modifies the adaptive $k$-swap mechanism originally designed for multi-agent
task allocation. The core idea is to approximate the NP-hard problem with an opportunistic and localized tour improvement heuristic by taking account of tour
constraints adaptively and flexibly, so that real-time solution can be obtained with small sacrifice on solution accuracy. 

To determine the number of the way points for navigation guidance in TSP, previous work~\cite{candes2009exact} has theoretically proven that a partially observed low-rank matrix could be perfectly recovered if the number of sampled entries $m$ obeys:
\begin{equation}
    \label{eq:sampled_cond}
        m\geq Cn^{1.2}r\log n,
\end{equation}
where $C$ is a positive numerical coefficient, $n = \max\left \{ n_1, n_2 \right \}$, and $r$ is the rank of the underlying matrix $\mathbf{M}$~\cite{candes2009exact}. Based on Eq.~(\ref{eq:sampled_cond}),
the placements of way points
can be defined
as:
\begin{equation}
    \label{eq:sample_num}
    N^{'}_{s} = \left \lfloor \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N^{'}_{s}$ represents the number of way points and $N$ is the number of observed map samples within each way point's local sensing range. 
Note that, in coverage planning scenarios, the robot can take observations in between any pair of successive sampling way points and may introduce additional observations. This implies we may want to reduce the number of sampled way points, 
and we do this by using a scale factor $\epsilon$, so that $N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor$, 
where $N_{s}$ is the number of sampled way points in TSP planning. 
We name this TSP based planning with different $\epsilon$ values as $TSP\_\epsilon$. 
Once a number of $N_{s}$ points are sampled, a fast and  near-shortest path will be formed using the adaptive \textit{k}-opt TSP solver and thereafter our robot could start the coverage mission by following the path. 




==> icra21-final/4_experiments.tex <==
\section{EXPERIMENTS}

To validate the proposed framework, we perform extensive simulation evaluations with a variety of complex maps. 

\subsection{Experimental Setups and Metrics Design}

To account for the sensor limitations as in robotics applications, we use two measurement patterns, \textit{Noisy Observation}~(NO) and \textit{Partial Observation}~(PO), for constructing the $\Omega$. NO means the observations are imperfect due to random noises (e.g., due to factors of environments/weathers such as snows, or sensor hardware limitations such as sparse and noisy measurements); 
PO means missed or uncovered regions which are typical in environmental mapping and monitoring scenarios. 

To quantitatively compare the two methods,  we use two evaluation metrics, \textit{total prediction accuracy}~(TPA), and \textit{computational time}~(CT). TPA indicates the correct entry matches (including the observed entries) between the entire predicted map and the ground-truth map while CT measures the required time for map prediction computation. 
In addition, we also evaluate the \textit{mapping convergence rate} during the coverage planning.


\subsection{Demonstration with Road Network Mapping}
\begin{figure}
  \centering
%   \subfigure[]
  	{\label{fig:road_image}\includegraphics[width=\linewidth]{figs/road_image.png}}
  \caption{\small \textit{Left}: road network displays linear dependent structures.  \textit{Right}: The road network is extracted where 
  the dark color represents the road while others are off-road places.
  } 
\label{fig:road_image}  
\end{figure}

\begin{figure} %\vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_comparison}\includegraphics[width=\linewidth]{figs/road_comparison.png}}
  \caption{\small Comparison between LRMC and BHM under NO~(first row) and PO~(second row) patterns, respectively. (a)\&(e)~Ground-truth maps. (b)\&(f)~Partially observed maps for NO and PO patterns. The missing parts are indicated in green patches. (c)\&(g)~Predicted maps from LRMC model. (d)\&(h)~Predicted maps from BHM.
  } \vspace{-10pt}
\label{fig:road_comparison}  
\end{figure}



We first demonstrate that our proposed LRMC method is able to perform map interpolation and extrapolation on a road network map extracted from an  urban environmental map, as shown in Fig.~\ref{fig:road_image}. 
The road surface can be detected by proximity sensors such as IR. We assume the robot is an aerial vehicle so that it can spot regions locally below it. 

The comparison of the two mapping methods on the urban road map under NO and PO patterns can be seen in Fig.~\ref{fig:road_comparison}. With NO pattern, both methods can generally predict the road network pattern~(topology), although BHM is more sensitive to the noises and thus fails to capture the exact road shape. On the other hand, with PO pattern, LRMC significantly outperforms BHM in the presence of multiple missing patches. 
Different from NO pattern, PO requires that the map prediction not only has interpolation capability, but also can perform slight extrapolation to reason the map structure within missing patches. 
LRMC leverages the linear dependency among the rows/columns of the map matrix and is able to predict the structure even multiple missing patches occur. In contrast, although BHM can capture local neighbouring spatial relationship by using kernelization, it is unable to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC. 

\subsection{Quantitative Comparison between LRMC and BHM}

We first generate 20 differing complex maze-like layouts/environments by using the Daedalus tool~\cite{daedalus}, and consider the TPA and CT statistical comparisons under NO and PO patterns for different values of $C$. 
The results are shown in Fig.~\ref{fig:us_acc_time_curve} and Fig.~\ref{fig:bus_acc_time_curve}. 
The trend of TPA and CT in different rank-valued maps %with different $C$ 
are shown in Fig.~\ref{fig:us_ranks_curve} for NO and Fig.~\ref{fig:bus_ranks_curve} for PO, respectively.

We first analyze the results for NO pattern. In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, it can be observed that 
LRMC could achieve a higher accuracy level. 
From Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we want to determine a proper scale of the coefficient $C$. We can think the coefficient $C$ is actually reflecting the number of observed map samples according to Eq.~(\ref{eq:sampled_cond}). 
In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we can see that TPA could reach a high level and stay stable when $C\geq 1.5$.
We then compare the CT performance as shown in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}. The result clearly distinguishes the two methods. The required computation time for LRMC is much lower than that of BHM. Given the size of the entire map~(matrix), the computational complexity of the LRMC algorithm~(SoftImpute~\cite{mazumder2010spectral}) we use is $O((m+n)r^2)$, where $m$ and $n$ are the dimensions and $r$ is the rank of the underlying ground-truth matrix. This means the LRMC model has a constant time complexity regardless of the number of observations. BHM is a logistic regression based method and has linear time complexity in terms of the number of observations. 

\begin{figure} 
  \centering
  	{\label{fig:us_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/us_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under NO pattern from 20 different mazes~(with different linear dependencies but the same rank). 
  } \vspace{-10pt}
\label{fig:us_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:us_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/us_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under NO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:us_ranks_curve}  
\end{figure}


\begin{figure}%[t] 
  \centering
  	{\label{fig:bus_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/bus_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under PO pattern from 20 different mazes~(with different linear dependencies but the same rank).  
  } \vspace{-10pt}
\label{fig:bus_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:bus_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/bus_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under PO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:bus_ranks_curve}  
\end{figure}

Note however, from Fig.~\ref{fig:us_acc_time_curve}-\textit{Right} we can see that the LRMC model has a better CT performance than constant time! The reason for this is the LRMC algorithm we use relies on SVD of the matrix. SVD is the most efficient for  dense matrices but not that efficient for sparse ones. In our case,   at first the number of observations can be small so the input matrix is a sparse one. 
The runtime benefit will actually  increase with more observations received, which is a significant feature for real-time robot mapping applications.  

In Fig.~\ref{fig:us_ranks_curve}, we compare the TPA and CT for environments with different ranks. It is clear to see in Fig.~\ref{fig:us_ranks_curve}-\textit{Left} that when the environment becomes more complex~(as the rank value increases), the accuracy of BHM decreases while LRMC maintains the same high-level prediction~(almost $100\%$). From the first row of Fig.~\ref{fig:road_comparison}, we can find BHM generally performs well but many minor discrepancies can be found along the road edges.  When the environment becomes complex, the number of edges increases and thus the minor errors accumulate and this results in the increase of the total map prediction error. The time performances~(Fig.~\ref{fig:us_ranks_curve}-\textit{Right}) of the two methods for different rank-valued maps show the same trend as in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}.

We then consider the results under PO pattern. Similar to what we have in the NO pattern, the TPA and CT results are shown in Fig.~\ref{fig:bus_acc_time_curve} and Fig.~\ref{fig:bus_ranks_curve}, respectively. The comparison results follow similar trends to the NO pattern. 

\subsection{Coverage Planning with Real-Time Map Prediction}

We investigate if the proposed map prediction can facilitate and improve existing environmental mapping and coverage planning methods. 
Our evaluations are based on three most prevalent strategies. 
The first planning method is the lawnmower (LM) planning: a simple but the most widely used coverage planning method in environmental surveying and monitoring.  Specifically, the traversal patterns and resolutions are pre-determined such that the whole area could be swept incrementally by the robot.
The second planning is the myopic planning (MP) which is typically based on greedy choices (or best-first actions). Here at each action step, a set of points are randomly sampled in all unexplored areas and the closest one to the robot is selected as the local goal. 
The third planning is the non-myopic customized $TSP\_\epsilon$ as described in Section~\ref{sect:plan}, 
where $\epsilon \in \left \{ 0.25,~0.5,~0.75 \right \}$.

\begin{figure*} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_tsp}\includegraphics[width=0.9\linewidth]{figs/road_tsp.png}}
  \caption{\small Environmental mapping of an urban road map using TSP\_{0.5}. The path is calculated by using an adaptive \textit{k}-opt TSP planner.
  In each of (a), (b), (c) and (d),  the \textit{Left} figure denotes the observed map while \textit{Right} is the predicted map using LRMC model, respectively. 
  } \vspace{-10pt}
\label{fig:road_tsp}  
\end{figure*}
% \begin{figure*} %\vspace{-3pt}
%   \centering
% %   \subfigure[]
%   	{\label{fig:terrain_tsp}\includegraphics[width=0.95\linewidth]{figs/terrain_tsp.png}}
%   \caption{\small {\color{blue} Environmental mapping of an terrain map using TSP\_{0.5}. The path~(yellow lines) is calculated by using an adaptive \textit{k}-opt TSP planner.
%   In each of (a), (b), (c) and (d),  the \textit{Left} figure denotes the observed map while \textit{Right} is the predicted map using LRMC model, respectively. }
%   } \vspace{-10pt}
% \label{fig:terrain_tsp}  
% \end{figure*}

\begin{figure}[t] 
  \centering
%   \subfigure[]
  	{\label{fig:coverage}\includegraphics[width=\linewidth]{figs/coverage.png}}
  \caption{\small Coverage convergence per action step for different coverage planning methods \textit{Left}: without real-time map prediction and \textit{Right}: with real-time map prediction.
  } \vspace{-10pt}
\label{fig:coverage}  
\end{figure}

The mapping process with non-myopic planning on the urban road network map is demonstrated in Fig.~\ref{fig:road_tsp}, where the real observed (sensed) map and corresponding predicted map from LRMC at four different action steps are presented. The results are consistent with that shown in Fig.~\ref{fig:road_comparison}.

To statistically evaluate the methods, we first consider the coverage planning with only raw observations but no map prediction. (As mentioned earlier, real-time predicted complete maps might not be available due to expensive computation cost in large environments.) The results are shown in Fig.~\ref{fig:coverage}-\textit{Left}, in which none of the listed methods could complete the map coverage within the given number of steps.
This also implies the necessity of real-time map prediction, 
and the results with map prediction are shown in Fig.~\ref{fig:coverage}-\textit{Right}. 
We can see that, 
within the same or less number of steps, nearly all of the planning methods could obtain a complete~(almost $100\%$) mapping coverage with real-time map prediction. 
In addition, the rate for coverage convergence is also remarkably improved for all of the listed coverage planning methods.

According to Fig.~\ref{fig:coverage}-\textit{Right}, among all the coverage planning methods, TSP\_$\epsilon$ methods significantly outperform other methods in terms of coverage convergence, although TSP based method can reach different completeness level as the value of $\epsilon$ varies. 
Empirically a larger value of $\epsilon$ can lead to more observations, a longer path~(and action steps), but also a better level of completeness (i.e., TSP\_{0.75}). A proper choice of $\epsilon$ value can give us a satisfactory trade-off between completeness and required action steps. 
Even with extremely restricted number of action steps~(i.e., less than 200), with a proper $\epsilon$, the TSP based methods can still achieve around $90\%$ coverage. The mapping results at different action steps by TSP\_{0.5} are shown in Fig.~\ref{fig:road_tsp}-(a), (b), (c) and (d), where we can see that our proposed method is able to perform map interpolation and extrapolation simultaneously on the fly during the execution of environmental mapping.

We also list the required number of action steps of all planning methods for different levels of completeness in Table~\ref{tb:coverage_comparison}. It is clear to see that with the proposed real-time LRMC map prediction all coverage planning methods can obtain a substantial improvement of coverage quality, and the required action steps at all listed completeness quantiles are remarkably reduced compared to the results without real-time map prediction.

\begin{table}\vspace{2pt}%[h]
\caption{\small Required number of action steps for varying levels of coverage completeness for different methods. The format for the entries indicates \textit{\# without real-time map prediction}~/~\textit{\# with real-time map prediction}, where `-' means the corresponding method fails to finish the respective completeness level.} %title of the table
\centering % centering table
{%\footnotesize
\begin{tabularx}{0.85\linewidth}{ccccc}%{c rrrrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & 20\% & 50\%  & 90\% & 100\% \\[0.5ex]
\hline % inserts single-line
LM  & 153 / 69 & - / 176 & - / 320 &  - / 356~(99\%)\\ [1ex]% Entering row contents
MP & 238 / 38 & - / 155 & - / 566 & - / -\\ [1ex]% [1ex] adds vertical space
TSP\_0.25  & 124 / 37 & - / 70 & - / \textbf{151} & - / - \\ [1ex]
TSP\_0.5  & 127 / 19 & - / 101 & - / 195 & - / \textbf{251}~(98\%)\\ [1ex]
TSP\_0.75  & 120  / \textbf{16} & - / \textbf{61} &- / 240 & - / \textbf{309} \\
\hline % inserts single-line
\end{tabularx}
}
\label{tb:coverage_comparison} \vspace{-10pt}
\end{table}










==> icra21-final/5_conclusions.tex <==
\section{CONCLUSIONS}
We consider the map prediction problem where the measurements are noisy, sparse and partially observed. We first show that many maps possess low-rank and incoherent structures. Then we propose to use LRMC to perform the map prediction. Our extensive experiments validate that the LRMC method can effectively perform map prediction (interpolation and extrapolation), and the LRMC method outperforms  state-of-the-art Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and could update the entire map in real-time. Lastly we show that the proposed real-time map prediction method can be easily combined with popular coverage planning methods and can significantly improve their coverage convergence rates.

==> icra21-new/0_abstract.tex <==
\begin{abstract}
%In this paper, with an assumption that the underlying map exhibits some special structures~(i.e., low-rank and incoherent structures), 
In many autonomous mapping tasks, the maps cannot be accurately constructed due to various reasons such as sparse, noisy, and partial sensor measurements.  
We propose a novel map prediction method built upon recent success of \textit{Low-Rank Matrix Completion}. The proposed map prediction is able to achieve both map interpolation and extrapolation on raw poor-quality maps with missing or noisy observations. 
We validate with extensive simulated experiments that the approach can achieve real-time computation for large maps, and the performance is superior to state-of-the-art map prediction approach --- Bayesian Hilbert Mapping in terms of mapping accuracy and computation time.
Then we demonstrate that with the proposed real-time map prediction framework, the coverage convergence rate~(per action step) for a set of representative coverage planning methods commonly used for environmental modeling and monitoring tasks can be significantly improved.

\end{abstract}

==> icra21-new/1_introduction.tex <==
\section{INTRODUCTION}
 
% One critical functionality for autonomous vehicles in environmental mapping is to obtain a feature map by leveraging the flexible mobility of the robotic platform and the measurement capability of sensors equipped on the vehicle. The obtained feature map not only feeds back the interested values to human operators, but also is crucial for subsequent planning and decision making. In this case, an accurate and fast map prediction is necessary for the robot to quickly update the global feature map in real-time. Almost all the sensors we use can be regarded inherently inaccurate due to many error factors in designing and manufacturing, and this can lead to severely degraded sensing quality, for example, the point cloud from a depth camera may contain many outliers and the one from a low-end LiDAR~(i.e., 16-beam) might be sparse. In addition, nearly all sensors have limited sensing range, which may result in large portions of the environment unobserved/missed by the robot. 
% %The limitations on sensors produce many impediments for obtaining a desired feature map, such as measurement noise and data missingness. 
% Hence the map prediction must base itself on those partially sampled~(observed) information to quickly predict an accurate map. The problem becomes even more challenging in large-scale scenarios, which are frequently encountered in most real applications.

Mapping is a critical functionality for an autonomous robot that needs to perform tasks in an initially unknown environment where an underlying map is constructed with onboard sensors. 
However, this can be challenging if the sensor measurements are inaccurate or if the environment can only be partially measured (sensed), which are commonly seen in autonomous mapping scenarios. 
For instance, the point clouds obtained from low-end proximity sensors (e.g., LiDAR, IR, Sonar) might be extremely sparse especially in spacious environments. The point clouds might also contain many outliers (noisy points). In addition, oftentimes a mapping robot cannot visit every spot of the environment and the traversed areas may only partially cover the space with only some small sub-regions being measured. 
Given the sparse, noisy, and partial observations, it is desirable that a complete map can be efficiently predicted to well match the ground-truth environment, which is the objective of this paper. 

More formally, the map prediction aims to predict map structure based on already known regions and could be categorized into two classes: interpolation and extrapolation. Map interpolation means given some observations (measurement samples), we want to predict the values \textit{in between} the sampled places;
Map extrapolation means given some observation samples (or map structures), we want to predict the map values \textit{beyond} the sampled places. 

\begin{figure} \vspace{5pt}
  \centering
%   \subfigure[]
  	{\label{fig:real}\includegraphics[width=\linewidth]{figs/real_examples.png}}
  \caption{\small Urban and residential environments reveal strong structured patterns, such as \textit{Left}: road (or street) network and \textit{Right}: buildings layout. These environments containing linear dependent structures can be modeled as low-rank-matrix maps.} 
\label{fig:real}  
\end{figure}


In this paper, we propose to use Low-Rank Matrix Completion~(LRMC) to leverage the ill-conditioned map data to predict the whole map. LRMC exploits some special structures, such as low rank~(or linear dependency) and incoherence hidden in underlying map to perform the prediction. Two examples that possess special patterns in urban/residential environments are shown in Fig.~\ref{fig:real}.
We first illustrate how a structured environmental map satisfies important assumptions required by LRMC model. Then we qualitatively demonstrate with an urban road network map that our proposed LRMC method outperforms state-of-the-art map prediction~(or regression) method -- Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian} which is a Bayesian extension of Hilbert Mapping~(HM)~\cite{ramos2016hilbert}, where the map prediction is treated as a kernelized logistic regression problem. BHM eliminates crucial regularization parameter tunning in HM, and outputs continuous maps where the occupancy value of any arbitrary point could be queried.

We conduct exhaustive simulations on a set of maze-like complex maps and quantitatively analyze that our proposed LRMC method is superior to BHM on the maps with varying linear patterns and different rank values. %in terms of mapping accuracy and computation time. you will repeat this immediately below.
Finally we combine the proposed real-time map prediction with representative coverage planning methods commonly used for environmental mapping and monitoring, and show that the mapping coverage convergence could be significantly improved with high mapping accuracy. 

% We first illustrate how a partially sampled urban building layout map fits into the LRMC model. Then we demonstrate that our proposed LRMC map prediction outperforms state-of-the-art map prediction~(or regression) method --- Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian} in terms of mapping accuracy and computation time performance. BHM is a Bayesian extension of Hilbert Mapping~(HM)~\cite{ramos2016hilbert}, where the map prediction is treated as a kernelized logistic regression problem. BHM eliminates crucial regularization parameter tunning in HM, and outputs continuous maps where the occupancy value of any arbitrary point could be queried.

% Our experiments show that BHM is incompetent in real-time applications but LRMC is able to maintain and update a global map very quickly. Finally we adopt some representative coverage planning methods commonly used for environmental mapping and show that with our proposed real-time map prediction, the coverage convergence could be significantly improved without loss of map accuracy. 

We summarize our contributions as follows:
\begin{itemize}
    \item 
    This is the first time to examine and report that many complex urban/residential environments possess low-rank and incoherent structure, and to apply Low-Rank Matrix Completion for map prediction based on sparse, noisy, and partially observed maps.
    \item
    Our proposed Low-Rank Matrix Completion based map prediction outperforms state-of-the-art map prediction method---Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and is able to perform prediction in real-time.
    \item
    We perform extensive simulations and demonstrate the remarkable effectiveness of our proposed method  which allows representative coverage planning methods to achieve faster mapping coverage convergence rates.  %commonly used in environmental mapping   can be substantially improved.
\end{itemize}


==> icra21-new/2_related_work.tex <==
\section{RELATED WORK}

%\textbf{Map Prediction.} 
% Map prediction 
% aims to predict map structure based on already revealed regions and could be categorized into two classes: \textit{interpolation} and \textit{extrapolation}. Map interpolation means given some map samples, we want to predict the values in between the sampled places. This type of mapping methods are 
Map prediction has been studied in occupancy mapping problems.  
Prevalent methods include Occupancy Girds Mapping~(OGM)~\cite{elfes1989using}, Gaussian Process Occupancy Mapping~(GPOM)~\cite{o2012gaussian, wang2016fast}, Hilbert Mapping~(HM)~\cite{ramos2016hilbert} and Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian}. Specifically, OGM belongs to discrete mapping and all grids are independent with each other. To eliminate the requirement of pre-defining discrete grids and the independence assumption in OGM, GPOM is proposed and used in many applications~\cite{jadidi2014exploration, jadidi2015mutual}. GPOM naturally captures the neighbouring information thanks to kernelization, but being a non-parametric model, it has a computation complexity of $O(n^3)$, where $n$ is the number of sampled data points. Combining various advantages of GPOM, a faster and simpler parametric model---HM and its Bayesian version, BHM, is proposed later to eliminate the cubical time complexity in GPOM.

Map extrapolation 
%indicates that given some map samples~(or structures), we want to predict the map values beyond the sampled places. This problem 
attracts increasing attention in recent years and almost all the current methods for map extrapolation are based on deep neural networks~(DNNs)~\cite{caley2019deep, pronobis2017learning, katyal2018occupancy, shrestha2019learned, saroya2020online, katyal2019uncertainty}. However, DNNs based methods require huge amount of data for training and hence are still limited in general applications. In this paper, we propose to use Low-Rank Matrix Completion to perform the map prediction. 
%We claim here and will show in later experiments that 
Our proposed LRMC based method falls in between the {interpolation} and {extrapolation} methods. Specifically, the LRMC method can not only well interpolate map values, but at the same time can  extrapolate the map structure beyond the explored areas. 

%\textbf{Low-Rank Matrix Completion.} 
In the past two decades, the Low-Rank Matrix Completion~(LRMC) problem has been well studied. The first theoretically guaranteed exact LRMC algorithm is proposed in~\cite{candes2009exact}, where any $n \times n$ incoherent matrices of rank $r$ are proven to be exactly recovered from $C n^{1.2}r\log n$ uniformly randomly sampled entries with high probability through solving a convex problem of nuclear norm minimization~(NNM). Subsequent works~\cite{candes2010power, chen2015incoherence, gross2011recovering, recht2011simpler} refine the provable completion results following the NNM based method. However, since all of the algorithms mentioned above are based on second order methods~\cite{liu2010interior}, they can become extremely expensive if the matrix dimension is large~\cite{cai2010singular}. Some first order based methods~\cite{cai2010singular, ji2009accelerated, mazumder2010spectral} are developed later. They solve the nuclear norm minimization problem in an iterative manner and rely on Singular Value Decomposition~(SVD) of matrices and are suited to large-scale matrix completion problems. In recent years, many other techniques are developed, such as coherent matrix completion~\cite{liu2017new, bhojanapalli2014universal, chen2014coherent}, non-linear matrix completion~\cite{eriksson2012high} and adaptive sampling~\cite{chen2015completing, eftekhari2018mc2}. %However, these methods require a special structure for the underlying matrix~(or sampling pattern) different than this work. %this work also requires, isn't it?
In this paper, we mainly employ the first order SVD based iterative method, such as~\cite{mazumder2010spectral} to solve the LRMC problem.


==> icra21-new/3_methodology.tex <==
\section{METHODOLOGY}
\label{sect:method}

% Map prediction exhibits the same form as the matrix completion if the map is represented by a matrix. Typical forms of map encountered in environmental monitoring include occupancy map, elevation map~(terrain map), and certain interested value 2D distribution map~(e.g., temperature distribution, $CO_2$ distribution, etc.). If the values are discretely distributed in a 2D plane, then the map will become a matrix. In this paper, we call those maps as feature maps and address the real-time prediction of a partially observed urban buildings layout map, in which the places identified~(for example, by an aerial vehicle from the air) as having buildings are treated as featured spaces, while other places as non-featured spaces. 

% In this section we first describe the definition of the general LRMC problem. Then we list two important assumptions required by LRMC model for the underlying feature map and we illustrate that maze-like environments satisfy those assumptions. Next, we give a reformulation of LRMC problem and lastly, we consider the incremental sampling process in environmental mapping scenarios and convert the map sampling problem into a way-points sampling. We also describe our proposed non-myopic planning method that is used to find an efficient path among the sampled way points.

\subsection{Problem Description}
Map prediction exhibits the same form as the matrix completion \cite{recht2009simpler} while a 2D map can be treated as a matrix. We propose to use LRMC as the map prediction method. LRMC is defined as completing a partially observed matrix $\tilde{\mathbf{M}}\in\mathbb{R}^{n_1\times n_2}$ whose part of entries are missing and the corresponding ground-truth matrix $\mathbf{M}$ has a low-rank and incoherent structures. Since the ground-truth rank is usually unknown, a typical way to complete $\tilde{\mathbf{M}}$ is to find a minimal rank matrix $\mathbf{X}^*$ that is consistent with $\tilde{\mathbf{M}}$ on the observed entries. A formal mathematical definition is:
\begin{equation}
    \label{eq:mc_1}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&rank(\mathbf{X})\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega,
    \end{aligned}
\end{equation}
where $\Omega \subset \left \{ 1, \cdots, n_1 \right \}\times \left \{ 1, \dots, n_2 \right \} $ is an index set of locations corresponding to the observed entries~($\left ( i, j \right )\in \Omega$ if $M_{ij}$ is observed). 

\subsection{Low-Rank and Incoherent Structures}
Two important assumptions for the underlying matrix $\mathbf{M}$ must be satisfied to guarantee the matrix completion results:
\begin{itemize}
    \item 
    $\mathbf{M}$ should be a low-rank matrix. A low-rank matrix implies its rank value is much smaller than its dimension and this structure enables the possibility to leverage linear dependencies among columns and/or rows of a matrix to predict missing entries~\cite{ongie2018tensor}. 
    \item
    $\mathbf{M}$ should be an incoherent matrix, which means the coherence of $\mathbf{M}$ is low. Suppose that a \textit{compact} SVD of a rank-r matrix $\mathbf{M}\in \mathbb{R}^{n_1\times n_2}$ is $\mathbf{M} = \mathbf{U}\Sigma\mathbf{V}^T$, where $\mathbf{U} \in \mathbb{R}^{n_1\times r}$ and $\mathbf{V}\in \mathbb{R}^{n_2\times r}$ are stacked left and right singular vectors of $\mathbf{M}$, while $\Sigma \in \mathbb{R}^{r\times r}$ is the diagonal matrix formed by a number of $r$ singular values of $\mathbf{M}$. The statistical leverage scores of $\mathbf{U}$ and $\mathbf{V}$ are defined by $\gamma_{U} = \underset{i\in \left \{ 1, \cdots, n_1 \right \}}{\text{max}}\left \| \mathbf{U}_{i,~:} \right \|^2_2$ and $\gamma_{V} = \underset{j\in \left \{ 1, \cdots, n_2 \right \}}{\text{max}}\left \| \mathbf{V}_{j,~ :} \right \|^2_2$, respectively, where $\mathbf{U}_{i,~:}$ and $\mathbf{V}_{j,~:}$ represent the $i^{th}$ and $j^{th}$ row of $\mathbf{U}$ and $\mathbf{V}$. Then the coherence of $\mathbf{M}$ is defined as:
    \begin{equation}
        \label{eq:coherence}
        \gamma_{M} = \max \left \{ \gamma_{U}, \gamma_{V} \right \}.
    \end{equation}
    The value of $\gamma_M$ is within $\left [ 0, 1 \right ]$ and an incoherent structure means the value of $\gamma_M$ is near 0. A small coherence value implies that the mass of values in the matrix will not concentrate on small portions, but spread out through the whole matrix.
\end{itemize}

Under the two conditions, the matrix $\tilde{\mathbf{M}}$ has been shown to be provably recoverable~\cite{candes2009exact}. Fig.~\ref{fig:mazes_1} and Table~\ref{tb:maze_prop} illustrate the trends of ranks and coherences of different structured environments which are similar to complex versions of either urban road networks or building layouts.
%urban layouts (outdoor) or building floor plans (indoor).   
We can observe that the typical structured environments have ranks below 100, which are significantly smaller compared to the original matrix dimensions which could be multiple magnitudes higher (e.g., $10^4$ or above). 
The trend of ranks also reflects the complexity of the environment, and the higher the rank is, the more complex the environment is.
Along with the rank values, we also list the coherence values computed by using Eq.~(\ref{eq:coherence}).
%The incoherence prevents the information of the row and column spaces of the matrix from being too concentrated in a few rows or columns.
Although the coherence increases proportionally to the rank, they all stay at a low level indicating high incoherence. %where we can be convinced they all are incoherent. 

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:mazes_1}\includegraphics[width=0.99\linewidth]{figs/mazes_with_ranks.png}}
  \caption{\small Maze environments with different ranks. %The value of 1.0 represents the featured space while 0.2 is non-featured space. Here we use 0 to represent missing parts, the color-map range from 0.2 (non-featured space) to 1.0 (featured space).
  } \vspace{-10pt}
\label{fig:mazes_1}  
\end{figure}

\begin{table}[h]

\caption{Matrix properties of maze environments} %title of the table
\centering % centering table
\begin{tabularx}{\linewidth}{YYYYYYY}%{c rrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & (a) & (b) & (c) & (d) & (e) & (f)\\
\hline % inserts single-line
Rank & 2 & 7 & 11 & 14 & 19 & 22\\ % Entering row contents
Coherence & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabularx}
\label{tb:maze_prop}
\end{table}


\subsection{Solving LRMC in Map Prediction}
\label{sect:static}

%We model the map prediction problem as a LRMC problem. 
To solve the LRMC problem, %Eq.~\eqref{eq:mc_1} gives a formal mathematical formulation for LRMC. 
the rank minimization problem in Eq.~(\ref{eq:mc_1}) is non-convex and NP-hard unfortunately, and hence of little practical use. An alternative way for Eq.~(\ref{eq:mc_1}) is to replace $rank(\mathbf{X})$ with $\left \| \mathbf{X} \right \|_*$, where $\left \| \mathbf{X} \right \|_*$ is the nuclear norm of $\mathbf{X}$, that is, the sum of sigular values of $\mathbf{X}$: $\left \| \mathbf{X} \right \|_* = \sum_{k=1}^{\min \left \{ n_1, n_2 \right \}}\sigma_k(\mathbf{X})$, where $\sigma_k(\mathbf{X})$ is the $k^{th}$ largest singular values of $\mathbf{X}$. The new formulation is:
\begin{equation}
    \label{eq:mc_2}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega.
    \end{aligned}
\end{equation}
The nuclear norm $\left \| \mathbf{X} \right \|_*$ is an effective convex relaxation to the rank objective and the optimization in Eq.~(\ref{eq:mc_2}) could be solved by semi-definite programming~\cite{laurent2014positive}.

Nevertheless, the optimizations in Eq.~(\ref{eq:mc_1}) and Eq.~(\ref{eq:mc_2}) aim to exactly recover the partially observed matrix, and this way was claimed as too rigid and may result in over-fitting~\cite{mazumder2010spectral}. A more robust way is to add a regularization parameter in Eq.~(\ref{eq:mc_2}):
\begin{equation}
    \label{eq:mc_3}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && \sum_{(i, j)\in \Omega}(X_{ij} - M_{ij})^2\leq \delta,
    \end{aligned}
\end{equation}
where $\delta \geq 0$ is a parameter regulating the training error tolerance. Equivalently Eq.~(\ref{eq:mc_3}) could be reformulated in a Lagrange form:
\begin{equation}
    \label{eq:mc_4}
    \begin{aligned}
        \mathbf{X}^* = \underset{\mathbf{X}}{\text{argmin}} \sum_{(i, j)\in \Omega} (X_{ij} - M_{ij})^2 + \lambda \left \|\mathbf{X} \right \|_{*},
    \end{aligned}
\end{equation}
where $\lambda$ is a regularization parameter controlling the nuclear norm. A SVD based iterative method proposed in~\cite{mazumder2010spectral} can be used to solve the Eq.~(\ref{eq:mc_4}).


\subsection{Mapping with Non-myopic Planner}
\label{sect:plan}

We are intrigued if the proposed map prediction can facilitate and improve existing environmental mapping and coverage methods. Popular planning paradigms include lawnmower mapping~\cite{li2019coverage, song2018varepsilon}, myopic (short-horizon) planning~\cite{khan2014greedy}, as well as non-myopic (long-horizon) planning~\cite{ kantaros2019asymptotically}. Lawnmower planning pursues complete spatial coverage, and myopic methods are oftentimes greedy schemes. The non-myopic approaches have been favored by many researchers for environmental mapping and monitoring~\cite{ma2016information, chen2019pareto}. Since non-myopic planners optimize paths over some horizon, we adopt and adapt the standard  \textit{Traveling Salesman Problem}~(TSP), which will be used in our evaluation in the experimental section. 

%With the predicted map, a non-myopic planer may be available to the mapping problem.
%The observation set $\Omega$ in LRMC typically is given at one-time. However, 
% In robotic environmental mapping scenarios, the observed/measured samples $\Omega$ are streamed along the robot traversal. 
% %cannot be given at one-time and the construction of $\Omega$ relies on the robot traversing the whole mapping space---this belongs to a coverage planning problem. 
% Therefore, we need to first determine a set of way points for future navigation guidance. 
%that need to be reached incrementally by the robot. A well-known efficient non-myopic planning method to find a path among a set of known locations is to solve the \textit{Traveling Salesman Problem}~(TSP). 
A TSP %definition in coverage planning 
can be defined as that, given the positions of a collection of way points, what is the shortest possible path of reaching each way point only once and eventually returning to the starting point. 
To efficiently solve the TSP, we extend our recently developed adaptive \textit{k}-opt method~\cite{ma2016adaptive} which exploits and modifies the adaptive $k$-swap mechanism originally designed for multi-agent
task allocation. The core idea is to approximate the NP-hard problem with an opportunistic and localized tour improvement heuristic by taking account of tour
constraints adaptively and flexibly, so that real-time solution can be obtained with small sacrifice on solution accuracy. 
%Different from existing \textit{k}-opt methods, the parameter $k$ in the adaptive \textit{k}-opt method is adjusted adaptively as the tour improvement proceeds. 

To determine the number of the way points for navigation guidance in TSP, previous work~\cite{candes2009exact} has theoretically proven that a partially observed low-rank matrix could be perfectly recovered if the number of sampled entries $m$ obeys:
\begin{equation}
    \label{eq:sampled_cond}
        m\geq Cn^{1.2}r\log n,
\end{equation}
where $C$ is a positive numerical coefficient, $n = \max\left \{ n_1, n_2 \right \}$, and $r$ is the rank of the underlying matrix $\mathbf{M}$~\cite{candes2009exact}. Based on Eq.~(\ref{eq:sampled_cond}),
%we consider a static environmental modeling scenario, i.e., static sensor placement problem, where the number of locations for placing sensors 
the placements of way points
can be defined %based on Eq.~(\ref{eq:sampled_cond}) 
as:
\begin{equation}
    \label{eq:sample_num}
    N^{'}_{s} = \left \lfloor \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N^{'}_{s}$ represents the number of way points and $N$ is the number of observed map samples within each way point's local sensing range. 
Note that, in coverage planning scenarios, the robot can take observations in between any pair of successive sampling way points and may introduce additional observations. This implies we may want to reduce the number of sampled way points, %as suggested by Eq.~(\ref{eq:sample_num}) 
and we do this by using a scale factor $\epsilon$, so that $N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor$, 
% \begin{equation}
%     \label{eq:new_sample_num}
%     N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor = \left \lfloor \epsilon \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
% \end{equation}
where $N_{s}$ is the number of sampled way points in TSP planning. 
We name this TSP based planning with different $\epsilon$ values as $TSP\_\epsilon$. 
Once a number of $N_{s}$ points are sampled, a fast and  near-shortest path will be formed using the adaptive \textit{k}-opt TSP solver and thereafter our robot could start the coverage mission by following the path. 
%where the $\epsilon$ is the scale factor in Eq.~(\ref{eq:new_sample_num}).




==> icra21-new/4_experiments.tex <==
\section{EXPERIMENTS}

%Through extensive evaluations, we demonstrate that the LRMC based map prediction is highly efficient and can significantly facilitate the coverage convergence in environmental mapping. 
% 
To validate the proposed framework, we perform extensive simulation evaluations with a variety of complex maps. 

\subsection{Experimental Setups and Metrics Design}

To account for the sensor limitations as in robotics applications, we use two measurement patterns, \textit{Noisy Observation}~(NO) and \textit{Partial Observation}~(PO), for constructing the $\Omega$. NO means the observations are imperfect due to random noises (e.g., due to factors of environments/weathers such as snows, or sensor hardware limitations such as sparse and noisy measurements); %sampled in entire mapping space at random. 
PO means missed or uncovered regions which are typical in environmental mapping and monitoring scenarios. 
%Then we quantitatively show that LRMC outperforms BHM and is able to facilitate coverage mapping process in general maze maps, which model the map types that possess linear dependency among spatial dimensions. Particularly for those maps satisfying low-rank and incoherent structures, the LRMC model has been proven to recover a partially observed map with theoretical guarantee. 

To quantitatively compare the two methods,  we use two evaluation metrics, \textit{total prediction accuracy}~(TPA), and \textit{computational time}~(CT). TPA indicates the correct entry matches (including the observed entries) between the entire predicted map and the ground-truth map while CT measures the required time for map prediction computation. 
In addition, we also evaluate the \textit{mapping convergence rate} during the coverage planning.


\subsection{Demonstration with Road Network Mapping}
\begin{figure}
  \centering
%   \subfigure[]
  	{\label{fig:road_image}\includegraphics[width=\linewidth]{figs/road_image.png}}
  \caption{\small \textit{Left}: road network displays linear dependent structures.  \textit{Right}: The road network is extracted where 
  %to obtain a binary map that is similar to maze maps, although the noises make the map not be rigorously low-rank. 
  the dark color represents the road while others are off-road places.
  } 
\label{fig:road_image}  
\end{figure}

\begin{figure} %\vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_comparison}\includegraphics[width=\linewidth]{figs/road_comparison.png}}
  \caption{\small Comparison between LRMC and BHM under NO~(first row) and PO~(second row) patterns, respectively. (a)\&(e)~Ground-truth maps. (b)\&(f)~Partially observed maps for NO and PO patterns. The missing parts are indicated in green patches. (c)\&(g)~Predicted maps from LRMC model. (d)\&(h)~Predicted maps from BHM.
  } \vspace{-10pt}
\label{fig:road_comparison}  
\end{figure}



We first demonstrate that our proposed LRMC method is able to perform map interpolation and extrapolation on a road network map extracted from an  urban environmental map, as shown in Fig.~\ref{fig:road_image}. 
The road surface can be detected by proximity sensors such as IR. We assume the robot is an aerial vehicle so that it can spot regions locally below it. 

The comparison of the two mapping methods on the urban road map under NO and PO patterns can be seen in Fig.~\ref{fig:road_comparison}. With NO pattern, both methods can generally predict the road network pattern~(topology), although BHM is more sensitive to the noises and thus fails to capture the exact road shape. On the other hand, with PO pattern, LRMC significantly outperforms BHM in the presence of multiple missing patches. 
Different from NO pattern, PO requires that the map prediction not only has interpolation capability, but also can perform slight extrapolation to reason the map structure within missing patches. 
LRMC leverages the linear dependency among the rows/columns of the map matrix and is able to predict the structure even multiple missing patches occur. In contrast, although BHM can capture local neighbouring spatial relationship by using kernelization, it is unable to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC. 

%From the second row of Fig.~\ref{fig:road_comparison}, we can see our LRMC model is able to achieve this and maintain the same accuracy level as itself under NO pattern. In contrast, BHM suffers from missing patches and perform even worse than itself under NO pattern.

% The results from both methods are shown in Fig.~\ref{fig:road_comparison}, in which the ground-truth map is the same as Fig.~\ref{fig:road_comparison}-(a). Under NO pattern~(first row), we observe both methods can achieve an exact or close-to-exact recovery. However, under PO pattern~(second row), LRMC significantly outperforms BHM in terms of the prediction accuracy. LRMC leverages the linear dependency among the row/columns of the map matrix and is able to predict the structure even multiple missing patches occur. In contrast, although BHM has a capacity to capture local neighbouring spatial relationship by using kernelization, it is unable to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC. 



%\footnote{\url{http://www.astrolog.org/labyrnth/daedalus.htm}}

% The goal of this paper is to demonstrate that a LRMC based map prediction is fast and efficient and can significantly facilitate the coverage convergence in urban environmental mapping. In this section, we first %show that the urban structured environments fit well into the LRMC model. Then we 
% conduct exhaustive comparison experiments between LRMC and BHM, under NO and PO, respectively; lastly we show that an outstanding coverage convergence rate improvement could be obtained if we equip commonly used coverage planning methods with our proposed LRMC real-time map prediction.

%\subsection{Assumptions Evaluation}

% To illustrate our considered structured environments satisfy the assumptions required by LRMC model, different maze maps with varying ranks are generated by Daedalus\footnote{\url{http://www.astrolog.org/labyrnth/daedalus.htm}} and are shown in Fig~\ref{fig:mazes_1}. Each map has a dimension of $20m \times 20m$ with a resolution of $0.1m$, which results in a matrix with dimension of $200\times 200$. The rank values are listed in Table~\ref{tb:maze_prop}. It is easy to observe that the value of rank basically reflects the complexity of the environment. The higher the rank is, the more complex the environment is. A typical urban building layout map~(see Fig.~\ref{fig:real}) has a rank below 100, which is significantly smaller compared to the original matrix dimension which could be multiple magnitudes higher (e.g., $10^4$ or above). 
% %would be similar to the maze with rank of 2, which is a very simple maze map. 
% %In this paper, we consider a more complicated environment that is similar to the maze with rank of 7~(as shown in Fig.~\ref{fig:mazes_1}-(b)). 
% %Compared with the dimension of 200, 7 is a much smaller value and therefore enables the corresponding matrix to be called as a low-rank matrix. Even the maze environment becomes super complex, such as the one shown in Fig.~\ref{fig:mazes_1}-(f), the rank value is still relatively small compared with the matrix dimension. 
% Along with the rank values, we also list the coherence value computed by using Eq.~(\ref{eq:coherence}) for each maze. Although the coherence increases proportionally to the rank, they all stay at a low-level where we can be convinced they all are incoherent. Hence we can conclude that maze environments generally possess the low-rank and low-coherence properties. 

% \begin{figure} \vspace{-3pt}
%   \centering
% %   \subfigure[]
%   	{\label{fig:mazes_1}\includegraphics[width=0.9\linewidth]{figs/mazes_with_ranks.png}}
%   \caption{\small Maze environments with different ranks. The value of 1.0 represents the featured space while 0.2 is non-featured space. Here we use 0 to represent missing parts, the color-map range from 0.2 (non-featured space) to 1.0 (featured space).
%   } \vspace{-10pt}
% \label{fig:mazes_1}  
% \end{figure}

% \begin{table}[t]
% \caption{Matric properties of maze environments} %title of the table
% \centering % centering table
% \begin{tabularx}{\linewidth}{YYYYYYY}%{c rrrrrrr} % creating eight columns
% \hline\hline %inserting double-line
% % Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
%   & (a) & (b) & (c) & (d) & (e) & (f)\\
% \hline % inserts single-line
% Rank & 2 & 7 & 10 & 15 & 18 & 23\\ % Entering row contents
% Coherence & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
% \hline % inserts single-line
% \end{tabularx}
% \label{tb:maze_prop}
% \end{table}


\subsection{Quantitative Comparison between LRMC and BHM}
% We first compare two map prediction methods, LRMC and BHM, on a static partially observed map.  That is, the observation set is given at one-time for the whole map. To account for the sensor limitations as in robotics applications, we use two measurement patterns, \textit{Noisy Observation}~(NO) and \textit{Partial Observation}~(PO), for constructing the $\Omega$, respectively. NO means the observations are imperfect due to random noises (e.g., due to factors of environments/weathers such as snows, or sensor hardware limitations such as sparse and noisy measurements); %sampled in entire mapping space at random. 
% PO means missed or uncovered regions which are typical in environmental mapping and monitoring scenarios. 
%there will be multiple regions are missed by the robot due to the limited sensing capability and PO models this situation.

% The results from both methods are shown in Fig.~\ref{fig:demo}, in which the ground-truth map is the same as Fig.~\ref{fig:demo}-(a). Under NO pattern~(first row), we observe both methods can achieve an exact or close-to-exact recovery. However, under PO pattern~(second row), LRMC significantly outperforms BHM in terms of the prediction accuracy. LRMC leverages the linear dependency among the row/columns of the map matrix and is able to predict the structure even multiple missing patches occur. In contrast, although BHM has a capacity to capture local neighbouring spatial relationship by using kernelization, it is unable to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC. 

%To further validate the effectiveness of the proposed LRMC map prediction method, 
% To quantitatively compare the two methods,  we use two evaluation metrics, \textit{total prediction accuracy}~(TPA), and \textit{computational time}~(CT). TPA indicates the correct entry matches (including the observed entries) between the entire predicted map and the ground-truth map while CT measures the required time for map prediction computation. 

We first generate 20 differing complex maze-like layouts/environments by using the Daedalus tool~\cite{daedalus}, and consider the TPA and CT statistical comparisons under NO and PO patterns for different values of $C$. 
%Then we generate %6 
%another set of differing environments with different rank values by Daedalus~\cite{daedalus} and again we apply the two map prediction methods and observe the trend of TPA and CT with different $C$. 
%The TPA and CT statistical comparisons under NO and PO patterns %for different values of $C$ 
The results are shown in Fig.~\ref{fig:us_acc_time_curve} and Fig.~\ref{fig:bus_acc_time_curve}. 
The trend of TPA and CT in different rank-valued maps %with different $C$ 
are shown in Fig.~\ref{fig:us_ranks_curve} for NO and Fig.~\ref{fig:bus_ranks_curve} for PO, respectively.

We first analyze the results for NO pattern. In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, it can be observed that 
%BHM has a bit faster accuracy convergence~(per $C$) but 
LRMC could achieve a higher accuracy level. 
%The high accuracy is known as an extremely important metric to evaluate the mapping performance.
%especially in mapping scenarios where the robot is subject to collision due to its limited distance to obstacles. %, although no significant difference in terms of accuracy can be found for the two methods. 
From Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we want to determine a proper scale of the coefficient $C$. We can think the coefficient $C$ is actually reflecting the number of observed map samples according to Eq.~(\ref{eq:sampled_cond}). 
%The higher the coefficient is, the more the observations are and the better the prediction is. 
In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we can see that TPA could reach a high level and stay stable when $C\geq 1.5$.
% below is too engineering and trivial, so removed.
%In real applications, the random sensing may show varying patterns each time and to be robust to this randomness, we select a value of 2.0 as a reference value for $C$ to achieve a desired prediction in the environments with a rank value of 7~(this is also reflected under PO pattern as shown in Fig.~\ref{fig:bus_acc_time_curve}-\textit{Left} later). 
We then compare the CT performance as shown in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}. The result clearly distinguishes the two methods. The required computation time for LRMC is much lower than that of BHM. Given the size of the entire map~(matrix), the computational complexity of the LRMC algorithm~(SoftImpute~\cite{mazumder2010spectral}) we use is $O((m+n)r^2)$, where $m$ and $n$ are the dimensions and $r$ is the rank of the underlying ground-truth matrix. This means the LRMC model has a constant time complexity regardless of the number of observations. BHM is a logistic regression based method and has linear time complexity in terms of the number of observations. 
Note however, from Fig.~\ref{fig:us_acc_time_curve}-\textit{Right} we can see that the LRMC model has a better CT performance than constant time! The reason for this is the LRMC algorithm we use relies on SVD of the matrix. SVD is the most efficient for  dense matrices but not that efficient for sparse ones. In our case,   at first the number of observations can be small so the input matrix is a sparse one. 
The runtime benefit will actually  increase with more observations received, which is a significant feature for real-time robot mapping applications.  
%and SVD may use some tricks to deal with the sparse matrix(i.e., fill in the missing parts with some well designed values before doing the decomposition). However, when the number of samples increases, the input matrix will be a dense one and the computation time for SVD decreases. 

% \begin{figure} %\vspace{-3pt}
%   \centering
% %   \subfigure[]
%   	{\label{fig:demo}\includegraphics[width=\linewidth]{figs/new_demo.png}}
%   \caption{\small First row: Map completion with \textit{Noisy Observation}. (a)~Ground-truth maze map. (b)~Partially observed map. The missing parts are indicated by green color (has value of $0.5$). (c)~The predicted map using LRMC model. (d)~The predicted map using BHM. Second row: Map completion with \textit{Partial Observations}. Note that color map is shared between subplots.
%   } \vspace{-10pt}
% \label{fig:demo}  
% \end{figure}

\begin{figure} 
  \centering
  	{\label{fig:us_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/us_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under NO pattern from 20 different mazes~(with different linear dependencies but the same rank). 
  } \vspace{-10pt}
\label{fig:us_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:us_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/us_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under NO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:us_ranks_curve}  
\end{figure}


\begin{figure}%[t] 
  \centering
  	{\label{fig:bus_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/bus_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under PO pattern from 20 different mazes~(with different linear dependencies but the same rank).  
  } \vspace{-10pt}
\label{fig:bus_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:bus_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/bus_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under PO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:bus_ranks_curve}  
\end{figure}



In Fig.~\ref{fig:us_ranks_curve}, we compare the TPA and CT for environments with different ranks. It is clear to see in Fig.~\ref{fig:us_ranks_curve}-\textit{Left} that when the environment becomes more complex~(as the rank value increases), the accuracy of BHM decreases while LRMC maintains the same high-level prediction~(almost $100\%$). From the first row of Fig.~\ref{fig:road_comparison}, we can find BHM generally performs well but many minor discrepancies can be found along the road edges.  When the environment becomes complex, the number of edges increases and thus the minor errors accumulate and this results in the increase of the total map prediction error. The time performances~(Fig.~\ref{fig:us_ranks_curve}-\textit{Right}) of the two methods for different rank-valued maps show the same trend as in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}.

We then consider the results under PO pattern. Similar to what we have in the NO pattern, the TPA and CT results are shown in Fig.~\ref{fig:bus_acc_time_curve} and Fig.~\ref{fig:bus_ranks_curve}, respectively. The comparison results follow similar trends to the NO pattern. 

% According to above discussions, we can conclude that under the experimental setup (map size, resolution, hinge points number, etc.) in this paper, although both methods can achieve a similar map prediction accuracy, BHM is incompetent in real-time applications but LRMC is able to maintain and update the global map very quickly.

% \begin{figure*}%[h!]
%   \centering
%     \includegraphics[width=\linewidth]{figs/tsp_results.png}
%   \caption{\small (a)~Ground-truth map for coverage planning. (b)~\textit{Left}: Real sensed map and \textit{Right}: predicted map in the middle of mapping with TSP\_{0.5}. (c)~\textit{Left}: Real sensed map and \textit{Right}: predicted map towards the ending of mapping with TSP\_{0.5}. }
%   \label{fig:tsp_results}
% \end{figure*}

\subsection{Coverage Planning with Real-Time Map Prediction}

We investigate if the proposed map prediction can facilitate and improve existing environmental mapping and coverage planning methods. 
Our evaluations are based on three most prevalent strategies. 
The first planning method is the lawnmower (LM) planning: a simple but the most widely used coverage planning method in environmental surveying and monitoring.  Specifically, the traversal patterns and resolutions are pre-determined such that the whole area could be swept incrementally by the robot.
The second planning is the myopic planning (MP) which is typically based on greedy choices (or best-first actions). Here at each action step, a set of points are randomly sampled in all unexplored areas and the closest one to the robot is selected as the local goal. 
%and a series of way-points are subsequently generated correspondingly. %The robot only takes the first way-point for execution.
The third planning is the non-myopic customized $TSP\_\epsilon$ as described in Section~\ref{sect:plan}, 
%We compare the coverage convergence performance~(per action step) of \textit{LM}, \textit{MP} and our proposed non-myopic planning --- $TSP\_\epsilon$, 
where $\epsilon \in \left \{ 0.25,~0.5,~0.75 \right \}$. %, on the same underlying maps.   Fig.~\ref{fig:tsp_results}-(a) demonstrates a scenario. The results of coverage convergence for different methods are shown in Fig.~\ref{fig:coverage}. 

%I mean only raw measurements, no post-processing(map prediction or map regression) is performed. Here I want to compare the environment modeling results with and without real-time map prediction and emphasize the use of real-time map prediction can really speedup the coverage convergence.




\begin{figure*} %\vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_tsp}\includegraphics[width=\linewidth]{figs/road_tsp.png}}
  \caption{\small Environmental mapping of an urban road map using TSP\_{0.5}. The path~(yellow lines) is calculated by using an adaptive \textit{k}-opt TSP planner. %The mapping results at one quarter, half, three quarters, and ending action step are shown in (a), (b), (c) and (d), 
  In each of (a), (b), (c) and (d),  the \textit{Left} figure denotes the observed map while \textit{Right} is the predicted map using LRMC model, respectively. 
  } \vspace{-10pt}
\label{fig:road_tsp}  
\end{figure*}

\begin{figure}[t] 
  \centering
%   \subfigure[]
  	{\label{fig:coverage}\includegraphics[width=\linewidth]{figs/coverage.png}}
  \caption{\small Coverage convergence per action step for different coverage planning methods \textit{Left}: without real-time map prediction and \textit{Right}: with real-time map prediction.
  } \vspace{-10pt}
\label{fig:coverage}  
\end{figure}

%We also show the advantage brought by LRMC to environmental modeling. 
The mapping process with non-myopic planning on the urban road network map is demonstrated in Fig.~\ref{fig:road_tsp}, where the real observed (sensed) map and corresponding predicted map from LRMC at four different action steps are presented. The results are consistent with that shown in Fig.~\ref{fig:road_comparison}. %The LRMC model can perform interpolation and extrapolation simultaneously during the execution of the mapping process and this could substantially accelerate coverage mapping progress and might be beneficial to decision makings for potential online adaptive planning.

To statistically evaluate the methods, we first consider the coverage planning with only raw observations but no map prediction. (As mentioned earlier, real-time predicted complete maps might not be available due to expensive computation cost in large environments.) The results are shown in Fig.~\ref{fig:coverage}-\textit{Left}, in which none of the listed methods could complete the map coverage within the given number of steps.
This also implies the necessity of real-time map prediction, 
%One may argue that some off-line methods can perform the prediction after the mission finishes. However, off-line methods lack flexibility and adaptivity to facilitate online decision making.
%One may argue that we can perform map prediction~(or regression) on the incomplete map after the mission finishes. This off-line map prediction does work to help human obtain a finer-resolution feature map, but it does also have problems if we want to monitor the space online or the planning algorithm require an online updated fine-grain map to make decisions in real-time. 
%Therefore, we have to consider to aid coverage planning with real-time map prediction, 
and the results with map prediction are shown in Fig.~\ref{fig:coverage}-\textit{Right}. 
We can see that, 
within the same or less number of steps, nearly all of the planning methods could obtain a complete~(almost $100\%$) mapping coverage with real-time map prediction. 
In addition, the rate for coverage convergence is also remarkably improved for all of the listed coverage planning methods. %compared to themselves without real-time map prediction. 
%We also claim that our proposed LRMC map prediction could be easily plugged with other planning methods that are not listed in this paper and facilitate their environmental mapping performance.

According to Fig.~\ref{fig:coverage}-\textit{Right}, among all the coverage planning methods, TSP\_$\epsilon$ methods significantly outperform other methods in terms of coverage convergence, although TSP based method can reach different completeness level as the value of $\epsilon$ varies. 
Empirically a larger value of $\epsilon$ can lead to more observations, a longer path~(and action steps), but also a better level of completeness (i.e., TSP\_{0.75}). A proper choice of $\epsilon$ value can give us a satisfactory trade-off between completeness and required action steps. 
%For example, if we have enough energy supply and pursue a well completed map, we should select a big value of $\epsilon$, such as 0.75. Otherwise, we can have a moderate magnitude $\epsilon$, like 0.25 to achieve an acceptable coverage ratio~(i.e., 90\%) if we have limited energy or constrained allowed action steps. 
Even with extremely restricted number of action steps~(i.e., less than 200), with a proper $\epsilon$, the TSP based methods can still achieve around $90\%$ coverage. The mapping results at different action steps by TSP\_{0.5} are shown in Fig.~\ref{fig:road_tsp}-(a), (b), (c) and (d), where we can see that our proposed method is able to perform map interpolation and extrapolation simultaneously on the fly during the execution of environmental mapping.

We also list the required number of action steps of all planning methods for different levels of completeness in Table~\ref{tb:coverage_comparison}. It is clear to see that with the proposed real-time LRMC map prediction all coverage planning methods can obtain a substantial improvement of coverage quality, and the required action steps at all listed completeness quantiles are remarkably reduced compared to the results without real-time map prediction.

\begin{table}\vspace{2pt}%[h]
\caption{\small Required number of action steps for varying levels of coverage completeness for different methods. The format for the entries indicates \textit{\# without real-time map prediction}~/~\textit{\# with real-time map prediction}, where `-' means the corresponding method fails to finish the respective completeness level.} %title of the table
\centering % centering table
{%\footnotesize
\begin{tabularx}{0.85\linewidth}{ccccc}%{c rrrrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & 20\% & 50\%  & 90\% & 100\% \\[0.5ex]
\hline % inserts single-line
LM  & 153 / 69 & - / 176 & - / 320 &  - / 356~(99\%)\\ [1ex]% Entering row contents
MP & 238 / 38 & - / 155 & - / 566 & - / -\\ [1ex]% [1ex] adds vertical space
TSP\_0.25  & 124 / 37 & - / 70 & - / \textbf{151} & - / - \\ [1ex]
TSP\_0.5  & 127 / 19 & - / 101 & - / 195 & - / \textbf{251}~(98\%)\\ [1ex]
TSP\_0.75  & 120  / \textbf{16} & - / \textbf{61} &- / 240 & - / \textbf{309} \\
\hline % inserts single-line
\end{tabularx}
}
\label{tb:coverage_comparison} \vspace{-10pt}
\end{table}










==> icra21-new/5_conclusions.tex <==
\section{CONCLUSIONS}
We consider the map prediction problem where the measurements are noisy, sparse and partially observed. We first show that many maps possess low-rank and incoherent structures. Then we propose to use LRMC to perform the map prediction. Our extensive experiments validate that the LRMC method can effectively perform map prediction (interpolation and extrapolation), and the LRMC method outperforms  state-of-the-art Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and could update the entire map in real-time. Lastly we show that the proposed real-time map prediction method can be easily combined with popular coverage planning methods and can significantly improve their coverage convergence rates. % in environmental mapping could be substantially improved. 

==> icra21/00_abstract.tex <==
\begin{abstract}

In this paper, with an assumption that the underlying feature map exhibits some special structures~(i.e., low-rank and incoherent structures), we propose a novel map prediction method building upon the theory of \textit{Low-Rank Matrix Completion}. The proposed map prediction is able to achieve both map interpolation and extrapolation in maze-like environments simultaneously.   We validate with extensive simulated experiments that our approach outperforms a state-of-the-art map prediction method --- Bayesian Hilbert Mapping in terms of mapping accuracy and computation time, and thus could be performed in real-time. Then we demonstrate that with our proposed real-time map prediction method, the coverage convergence~(per action step) for some typical coverage planning methods commonly used for environmental monitoring tasks can be significantly improved.

\end{abstract}

==> icra21/01_introduction.tex <==
\section{INTRODUCTION}
One critical functionality for autonomous vehicles in environmental monitoring is feature mapping, which aims to obtain a feature map~(e.g., terrain map, building layout map, and chemical concentration map) by leveraging the flexible mobility of the robotic platform and the measurement capability of the sensors equipped on the vehicle. The obtained feature map not only feeds back the interested values to human operators, but also is crucial for planning to make decisions if a highly intelligent autonomy is required. In this case, an accurate and fast map prediction is necessary for the robot to quickly update the global feature map in real-time. Almost all the sensors we use can be regarded inherently inaccurate due to many error factors in designing and manufacturing, and this can lead to severely degraded sensing quality, for example, the point cloud from a depth camera may contain many outliers and the one from a low-end LiDAR~(i.e., 16-beam) might be sparse. In addition, nearly all sensors have limited sensing range, which may result in large portions of the environment unobserved/missed by the robot. The limitations on sensors produce many impediments in obtaining a desired feature map, such as measurement noise and data missingness. Hence the map prediction has to quickly predict an accurate map based on those partially sampled~(observed) information. The problem becomes even more challenging in large-scale scenarios, which are frequently encountered in most real applications.

In this paper, we propose to use Low-Rank Matrix Completion~(LRMC) to leverage the partially observed map information to predict the whole feature map in an urban building layout monitoring task~(where we assume no trees or other objects occluding the buildings). We first model the urban building layout map as a maze map and carefully illustrate how the partially sampled maze environments fit into the LRMC model. Then we demonstrate that our proposed LRMC map prediction outperforms some state-of-the-art map prediction~(or regression) method, such as Bayesian Hilbert Mapping~(BHM) in terms of mapping accuracy and computation time performance. Given the experimental setups in this paper, our experiments show that BHM is far from being used in real-time applications but the LRMC is able to maintain and update the global map very quickly. Finally we adopt some representative coverage planning methods commonly used for environmental monitoring and show that with our proposed real-time map prediction, the coverage convergence(per action step) could be significantly improved without loss of map accuracy. 

We summarize our contributions as follows:
\begin{itemize}
    \item 
    We are the first to examine and illustrate that maze-like environments possess low-rank and incoherent structure.
    \item
    We are the first to apply Low-Rank Matrix Completion to predict the partially observed maze environments.
    \item
    Our proposed Low-Rank Matrix Completion based map prediction outperforms another state-of-the-art mapping method---Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and is able to perform prediction in real-time.
    \item
    We provide intensive simulated experiments and demonstrate the outstanding effectiveness of our proposed method and we also show that with our proposed real-time map prediction, the coverage convergence rate~(per action step) of some coverage planning methods commonly used in environmental monitoring can be substantially improved.
\end{itemize}


==> icra21/02_related_work.tex <==
\section{RELATED WORK}

\textbf{Map Prediction.} Map prediction aims to predict map structure based on already revealed regions and could be categorized into two classes: \textit{interpolation} and \textit{extrapolation}. Map interpolation means given some map samples, we want to predict the values in between the sampled places. This type of mapping methods are usually seen in occupancy mapping field, such as Occupancy Girds Mapping~(OGM)~\cite{elfes1989using}, Gaussian Process Occupancy Mapping~(GPOM)~\cite{o2012gaussian, wang2016fast}, Hilbert Mapping~(HM)~\cite{ramos2016hilbert} and Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian}. OGM divides the world into fixed-size grids and apply a Bayes filter to predict the occupancy values of the environment with an assumption that all the grids are independent with each other. To eliminate the requirement of pre-defining a discrete grid and the independent assumption in OGM, GPOM is proposed and used in many applications~\cite{jadidi2014exploration, jadidi2015mutual}. GPOM naturally captures the neighbouring information thanks to kernelization, but being a non-parametric model, it has a computation complexity of $O(n^3)$, where $n$ is the number of sampled data points. Bringing all the advantages of GPOM, a faster and simpler parametric model---HM and its Bayesian version, BHM, are proposed later. HM/BHM treats the map prediction as a kernelized logistic regression and has a linear time complexity. 

Map extrapolation indicates that given some map samples~(or structures), we want to predict the map values beyond the sampled places. This problem attracts increasing attention in recent years and almost all the current methods for map extrapolation are based on deep neural networks~(DNNs)~\cite{caley2019deep, pronobis2017learning, katyal2018occupancy, shrestha2019learned, saroya2020online, katyal2019uncertainty}. However, DNNs based methods require huge amount of data for training and hence still be very problematic. In this paper, we propose to use Low-Rank Matrix Completion to perform the map prediction. We claim here and will show in later experiments that our proposed LRMC based method fall in between the \textit{interpolation} and \textit{extrapolation} methods. Specifically, the LRMC method can not only well interpolate map values, but at the same time can weakly extrapolate the map structure beyond the explored areas in real-time. 

\textbf{Low-Rank Matrix Completion.} In the past two decades, the Low-Rank Matrix Completion~(LRMC) problem has been widely studied. The first theoretically guaranteed exact LRMC algorithm is proposed in~\cite{candes2009exact}, where any $n \times n$ incoherent matrices of rank r are proven to be exactly recovered from $C n^{1.2}r\log n$ uniformly randomly sampled entries with high probability through solving a convex problem of nuclear norm minimization~(NNM). Subsequent works~\cite{candes2010power, chen2015incoherence, gross2011recovering, recht2011simpler} refine the provable completion results following the NNM based method. However, since all of the algorithms mentioned above are based on second order methods~\cite{liu2010interior}, they can become extremely expensive if the matrix dimension is large~\cite{cai2010singular}. Some first order based methods~\cite{cai2010singular, ji2009accelerated, mazumder2010spectral} are developed to overcome the limitations of the second-order based methods. They solve the nuclear norm minimization problem in an iterative manner and rely on Singular Value Decomposition~(SVD) of matrices and are suited to large-scale matrix completion problems. Many other aspects of matrix completion could be found in~\cite{hastie2015matrix, liu2017new, eriksson2012high, bhojanapalli2014universal, chen2015completing, chen2014coherent, eftekhari2018mc2}.

==> icra21/03_preliminaries.tex <==
\section{PRELIMINARIES}

\subsection{Low-Rank Matrix Completion}
\textit{Low-Rank Matrix Completion} is defined as completing a partially observed matrix $\tilde{\mathbf{M}}\in\mathbb{R}^{n_1\times n_2}$ whose part of entries are missing and the corresponding ground-truth matrix $\mathbf{M}$ has a low-rank structure, which indicates $rank(\mathbf{M})\ll \min \left \{ n_1, n_2 \right \}$. Since the ground-truth rank is unknown at most times, a typical way to complete $\tilde{\mathbf{M}}$ is to find a minimal rank matrix $\mathbf{X}^*$ that is consistent with $\tilde{\mathbf{M}}$ on the observed entries. A formal mathematical definition is:
\begin{equation}
    \label{eq:mc_1}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&rank(\mathbf{X})\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega,
    \end{aligned}
\end{equation}
where $\Omega \subset \left \{ 1, \cdots, n_1 \right \}\times \left \{ 1, \dots, n_2 \right \} $ is an index set of locations corresponding to the observed entries~($\left ( i, j \right )\in \Omega$ if $M_{ij}$ is observed). Unfortunately, the rank minimization problem in Eq.~(\ref{eq:mc_1}) is non-convex and NP-hard, and hence of little of practical use. An alternative way for Eq.~(\ref{eq:mc_1}) is to replace $rank(\mathbf{X})$ with $\left \| \mathbf{X} \right \|_*$, where $\left \| \mathbf{X} \right \|_*$ is the nuclear norm of $\mathbf{X}$, that is, the sum of sigular values of $\mathbf{X}$: $\left \| \mathbf{X} \right \|_* = \sum_{k=1}^{\min \left \{ n_1, n_2 \right \}}\sigma_k(\mathbf{X})$, where $\sigma_k(\mathbf{X})$ is the $k^{th}$ largest singular values of $\mathbf{X}$. The new formulation is:
\begin{equation}
    \label{eq:mc_2}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega.
    \end{aligned}
\end{equation}
The nuclear norm $\left \| \mathbf{X} \right \|_*$ is an effective convex relaxation to the rank objective and the optimization in Eq.~(\ref{eq:mc_2}) could be solved in semidefinite programming.

However, the optimizations in Eq.~(\ref{eq:mc_1}) and Eq.~(\ref{eq:mc_2}) aim to exactly recover the partially observed matrix, and this way was claimed as too rigid and may result in over-fitting~\cite{mazumder2010spectral}. A more robust way is to add a regularization parameter in Eq.~(\ref{eq:mc_2}):
\begin{equation}
    \label{eq:mc_3}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && \sum_{(i, j)\in \Omega}(X_{ij} - M_{ij})^2\leq \delta,
    \end{aligned}
\end{equation}
where $\delta \geq 0$ is a parameter regulating the training error tolerance. Equivalently Eq.~(\ref{eq:mc_3}) could be reformulated in a Lagrange form:
\begin{equation}
    \label{eq:mc_4}
    \begin{aligned}
        \mathbf{X}^* = \underset{\mathbf{X}}{\text{argmin}} \sum_{(i, j)\in \Omega} (X_{ij} - M_{ij})^2 + \lambda \left \|\mathbf{X} \right \|_{*},
    \end{aligned}
\end{equation}
where $\lambda$ is a regularization parameter controlling the nuclear norm.


\subsection{Assumptions for Completion Guarantee}
Three important assumptions for the underlying matrix $\mathbf{M}$ and the observation set $\Omega$ must be satisfied to guarantee the matrix completion results according to~\cite{candes2009exact}:
\begin{itemize}
    \item 
    $\mathbf{M}$ should be a low-rank matrix. A low-rank matrix implies its rank value is much smaller than its dimension and this structure enables the possibility to leverage linear dependencies among columns and/or rows of a matrix to impute missing entries~\cite{ongie2018tensor}. 
    \item
    $\mathbf{M}$ should be an incoherent matrix, which means the coherence of $\mathbf{M}$ is low. Suppose that a \textit{compact} SVD of a rank-r matrix $\mathbf{M}\in \mathbb{R}^{n_1\times n_2}$ is $\mathbf{M} = \mathbf{U}\Sigma\mathbf{V}^T$, where $\mathbf{U} \in \mathbb{R}^{n_1\times r}$ and $\mathbf{V}\in \mathbb{R}^{n_2\times r}$ are stacked left and right singular vectors of $\mathbf{M}$, while $\Sigma \in \mathbb{R}^{r\times r}$ is the diagonal matrix formed by the $r$ singular values of $\mathbf{M}$. The statistical leverage scores of $\mathbf{U}$ and $\mathbf{V}$ are defined by $\gamma_{U} = \underset{i\in \left \{ 1, \cdots, n_1 \right \}}{\text{max}}\left \| \mathbf{U}_{i,~:} \right \|^2_2$ and $\gamma_{V} = \underset{j\in \left \{ 1, \cdots, n_2 \right \}}{\text{max}}\left \| \mathbf{V}_{j,~ :} \right \|^2_2$, respectively, where $\mathbf{U}_{i,~:}$ and $\mathbf{V}_{j,~:}$ represent the $i^{th}$ and $j^{th}$ row of $\mathbf{U}$ and $\mathbf{V}$. Then the coherence of $\mathbf{M}$ is defined as:
    \begin{equation}
        \label{eq:coherence}
        \gamma_{M} = \max \left \{ \gamma_{U}, \gamma_{V} \right \}.
    \end{equation}
    \item
    The observation set $\Omega$ should be randomly uniformly sampled and the number of the sampled entries $m$ should obey: 
    \begin{equation}
        \label{eq:sampled_cond}
            m\geq Cn^{1.2}r\log n,
    \end{equation}
    where $C$ is some positive numerical coefficient, $n = \max\left \{ n_1, n_2 \right \}$, and $r$ is the rank of the underlying matrix $\mathbf{M}$~\cite{candes2009exact}.
\end{itemize}




==> icra21/04_map_prediction.tex <==
\section{MAP PREDICTION}
\label{sec:map_completion}

\begin{table*}[t]
\caption{Matric properties of maze environments} %title of the table
\centering % centering table
\begin{tabular}{c rrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & (a) & (b) & (c) & (d) & (e) & (f)\\
\hline % inserts single-line
Rank & \vline & 2 & 7 & 10 & 15 & 18 & 23\\ % Entering row contents
Coherence & \vline & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabular}
\label{tb:maze_prop}
\end{table*}

Map completion exhibits the same form as the matrix completion if the map is represented by a matrix. Typical forms of map encountered in environmental monitoring include occupancy map, elevation map~(terrain map), and certain interested value 2D distribution map~(e.g., temperature distribution, $CO_2$ distribution, etc.). If the values are discretely distributed in a 2D plane, then the map will become a matrix. In this paper, we call those maps as feature maps and address the real-time prediction of a partially observed urban buildings layout map, in which the places identified~(by an aerial vehicle from the air) as having buildings are treated as featured spaces, while other places as non-featured spaces. In this section we show that a maze-like feature map satisfies the assumptions of the LRMC model and how the LRMC model performs the prediction given a partially revealed maze map.

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:mazes_1}\includegraphics[width=0.9\linewidth]{figs/mazes_with_ranks.png}}
  \caption{\small Maze environments with different ranks. The value of 1.0 represents the featured space while 0.2 is the non-featured space~(the reason for using 0.2 is in LRMC model, we need to fill missing parts with 0, then to distinguish the known parts and missing parts, we use some non-zero value to represent the non-featured space).
  } \vspace{-10pt}
\label{fig:mazes_1}  
\end{figure}

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:demo}\includegraphics[width=\linewidth]{figs/new_demo.png}}
  \caption{\small First row: Map completion with \textit{Uniform Sampling}. (a)~Ground-truth maze map. (b)~Partially observed map. The missing parts are indicated by value of $0.5$~(indicated by green color). (c)~The predicted map using LRMC model. Second row: Map completion with \textit{Blocked Uniform Sampling}. The colors have the same meaning with the first row.
  } \vspace{-10pt}
\label{fig:demo}  
\end{figure}

Different maze maps with varying ranks are generated by Daedalus\footnote{\url{http://www.astrolog.org/labyrnth/daedalus.htm}} and are shown in Fig~\ref{fig:mazes_1}. Each map has a dimension of $20m \times 20m$ with a resolution of $0.1m$, which results in a matrix with dimension of $200\times 200$. The rank values are listed in Table~\ref{tb:maze_prop}. It is easy to observe that the value of rank basically reflects the complexity of the matrix. The higher the rank is, the more complex the environment is. A typical urban building layout map would be similar to the maze with rank of 7 (as shown in Fig.~\ref{fig:mazes_1}-(b)), which is also the rank parameter we adopt in this paper. Compared with the dimension of 200, 7 is a much smaller value and therefore enables the corresponding matrix to be called as a low-rank matrix. Even the maze environment becomes super complex, such as the one shown in Fig.~\ref{fig:mazes_1}-(f), the rank value is still relatively small compared with the matrix dimension. Along with the rank values, we also list the coherence value for each maze matrix using the Eq.~(\ref{eq:coherence}). Although the coherence increases proportionally to the rank, they all stay at a low-level where we can be convinced they all are incoherent. Hence we can conclude that maze environments generally possess the low-rank and low-coherence properties required by the LRMC model. 

The sensors used in environmental monitoring are usually interfered with exogenous factors~(such as wind disturbance, magnetic field, light conditions, etc.) and endogenous factors~(such as manufacturing limitations, installation error, etc.). Consequently, the raw measurements~(samples) from sensors could be noisy and in many cases be sparse. In this section, we demonstrate the proposed LRMC based algorithm is robust to the degraded sensing measurements by considering two sampling patterns in a static map prediction scenario: \textit{Uniform Sampling}~(US) and \textit{Blocked Uniform Sampling}~(BUS). US means the observations are uniformly sampled in the mapping space at random. On the other hand, in many real scenarios, there will be some blocks are missed by the robot due to the limited sensing capability and there will be multiple regions where no any data point is sampled and BUS models this situation. Examples for map completion on a partially observed maze map with two sampling patterns are shown in Fig.~\ref{fig:demo}. Note that throughout this paper, we adopt the  SoftImpute~\cite{mazumder2010spectral} for implementing the LRMC model.

In both examples, we randomly select less-half observations and apply the LRMC model to the partial matrix. The evaluation metric we use is called \textit{total prediction accuracy}~(TPA), which indicates the correct entry matches~(including the already observed parts) between the entire predicted maze and the ground-truth maze and reflects the entire prediction completeness. The TPA results for two sampling patterns are shown in Table~\ref{tb:exam_stat}. It is clear that even with less than half of revealed/observed entries, the LRMC model could achieve an exact~(or near-exact) correct predictions. However, it is still unclear at least exactly how many samples we need to achieve an exact recovery.

\begin{table}%[h]
\caption{Statistics for Fig.~\ref{fig:demo}} %title of the table
\centering % centering table
\begin{tabular}{c rrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & US & BUS\\
\hline % inserts single-line
Revealed percentage~(\%) & \vline & 40.67 & 40.67\\ % Entering row contents
TPA~(\%) & \vline & 100.0 & 95.72\\
\hline % inserts single-line
\end{tabular}
\label{tb:exam_stat}
\end{table}

\begin{figure} \vspace{-6pt}
  \centering
%   \subfigure[]
  	{\label{fig:mc_curves}\includegraphics[width=\linewidth]{figs/mc_curves.png}}
  \caption{\small TPA results with different values of coefficient $C$ under \textit{Left}: US pattern and \textit{Right}: BUS pattern.
  } \vspace{-10pt}
\label{fig:mc_curves}  
\end{figure}

Some of previous works~\cite{candes2009exact} has theoretically proven a partially observed low-rank matrix could be perfectly recovered if the number of sampled entries $m$ obeys the Eq.~(\ref{eq:sampled_cond}). Although it seems that the number of observation samples are theoretically lower bounded, it is still difficult to determine the exact value of the $m$ due to the existence of $C$. To determine a proper scale of the coefficient $C$, we generate 20 maze environments with the same rank of 7 and apply the LRMC model to different partially observed mazes under US and BUS patterns and unveil the relationship between the coefficient $C$ and TPA. For each value of $C$ we compute a mean and standard deviation for TPA and the results are shown in Fig.~\ref{fig:mc_curves}.

We can think the coefficient $C$ is actually reflecting the number of observed entries according to Eq.~(\ref{eq:sampled_cond}). The higher the coefficient is, the more the observations are and the better the prediction is. From Fig.~\ref{fig:mc_curves}, we can see that for both sampling patterns, the TPA could reach a high level and stay stable when $C\geq 1.5$. Since in real applications, the sampling shows undeterminitic patterns and to be robust to this randomness, we select a value that is bigger than 1.5, 2.0 as a reference value for $C$ to achieve a desired prediction in the selected maze environment. This reference value will guide the later experiments in this paper.



==> icra21/05_experiments.tex <==
\section{EXPERIMENTS}
The goal of this paper is to demonstrate that a LRMC based map prediction is efficient and fast and can significantly facilitate the coverage convergence in environmental monitoring. We have shown that the maze-like environments fit well into the LRMC model. We want to understand in a further step how the model behaves compared to other state-of-the-art map prediction method, i.e., Bayesian Hilbert Mapping~(BHM) in terms of TPA as well as computation time. We also want to know how commonly used coverage planning methods can benefit from real-time map prediction. In this section, we firstly conduct exhaustive comparison experiments between LRMC and BHM, under US and BUS, respectively; then we show that an outstanding coverage convergence improvement could be obtained if we equip commonly used coverage planning methods with our proposed LRMC real-time map prediction.

\subsection{Comparison between LRMC and BHM}
We compare two map prediction methods, LRMC and BHM, on a static partially observed map, that is, the sampling is given at one-time for the whole map. The ground-truth map is the same as Fig.~\ref{fig:demo}-(a) and the map size parameters are set as the ones in Section.~\ref{sec:map_completion}. We set the value of $C$ as $2.0$~(as discussed in Section.~\ref{sec:map_completion}) and the results from both methods are shown in Fig.~\ref{fig:comparison_1}. Under US pattern, we observe both methods can achieve an exact~(or almost) recovery~(as shown in the first row of Fig.~\ref{fig:comparison_1}). However, under BUS pattern, LRMC significantly outperforms BHM in terms of the prediction accuracy~(as shown in the second row of Fig.~\ref{fig:comparison_1}). LRMC leverages the linear dependency among the row/columns of the map matrix and is able to predict the structure even multiple blocks of missing occur. In contrast, although BHM has a capacity to capture local neighbouring spatial relationship by using kernelized features, it lacks the ability to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC in maze-like environments. To validate the effectiveness of our proposed LRMC map prediction method, we consider the comparisons under both US and BUS patterns. The evaluation metrics we use in this section is TPA and \textit{computational time}~(CT). 

Under US pattern, we first generate 20 maze environments with the same rank value of 7 and apply LRMC and BHM to the 20 mazes and collect the TPA and CT values per different values of $C$~(as shown in Fig.~\ref{fig:us_acc_time_curve}). Then we generate 6 maze environments with different ranks values and again we apply the two map prediction methods and observe the trend of TPA and CT with different $C$~(as shown in Fig.~\ref{fig:us_ranks_curve}). 

In Fig.~\ref{fig:us_acc_time_curve}, it can be observed that BHM has a bit faster accuracy convergence~(per $C$) but LRMC could achieve a higher accuracy level, although no significant difference in terms of accuracy can be found for the two methods. On the other hand, CT performance clearly distinguish the two and the required computation time for LRMC is mush lower than that of BHM. Given the size of the entire map~(matrix), the computational complexity of the LRMC algorithm we use, SoftImpute~\cite{mazumder2010spectral}, is $O((m+n)r^2)$, where $m$ and $n$ are the dimensions and $r$ is the rank of the underlying ground-truth matrix. This means the LRMC model has a constant time complexity in terms of number of samples. BHM is a logistic regression based method and has linear time complexity. Therefore, from the theoretical analysis of computational complexity, we can see that LRMC is better than BHM. However, from Fig.~\ref{fig:us_acc_time_curve}, our experiments show that LRMC model has a better time performance than constant one! The reason for this is the LRMC algorithm we use relies on SVD of the matrix. SVD is friendly to dense matrices but not that efficient for sparse matrices. In our case, when the number of samples is small, the input matrix is a sparse one and SVD may use some tricks to deal with the sparse matrix(i.e., fill in the missing parts with some well designed values before doing the decomposition). However, when the number of samples increases, the input matrix will be a dense one and the computation time for SVD decreases. According to Fig.~\ref{fig:us_acc_time_curve}, we can conclude that under the experimental setup(map size, resolution, hinge points number, etc.) in this paper, BHM is far from being used in real-time applications but LRMC is able to maintain and update the global map very quickly.

In Fig.~\ref{fig:us_ranks_curve}, we compare the TPA/CT per $C$ for mazes with different ranks. It is clear to see that when the environment becomes more complex~(as the rank value increases), the accuracy of BHM decreases while LRMC maintain the same high-level prediction(almost $100\%$). From the first row of Fig.~\ref{fig:comparison_1}, we can find BHM generally performs very well but many minor errors can be found along the edges. When the environment becomes complex, the number of edges increases and thus the minor errors accumulate and this results in the increase of the total map prediction error.

Under BUS pattern, similar to what we have in US pattern, the TPA/CT per $C$ results for mazes with the same rank and different ranks are shown in Fig.~\ref{fig:bus_acc_time_curve} and Fig.~\ref{fig:bus_ranks_curve}, respectively. The comparison results are basically the same as we discussed under US pattern.

% \begin{figure}%[h!]
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{figs/pls_coverage.png}
%     \caption{}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%     \includegraphics[width=\linewidth]{figs/dls_coverage.png}
%     \caption{}
%   \end{subfigure}
%   \caption{\small Coverage convergence of different methods for (a)~PLS mode and (b)~DLS mode.}
%   \label{fig:coverage}
% \end{figure}



\begin{figure}
  \centering
%   \subfigure[]
  	{\label{fig:comparison_1}\includegraphics[width=\linewidth]{figs/comparison_1.png}}
  \caption{\small Map prediction comparison between LRMC and BHM. \textit{First row}: With US pattern. (a)~Partially observed map. Predicted map results from (b)~LRMC and (c)~BHM. \textit{Second row}: With BUS pattern. (d)~Partially observed map. Predicted map results from (e)~LRMC and (f)~BHM.  } \vspace{-10pt}
\label{fig:comparison_1}  
\end{figure}

\begin{figure} 
  \centering
  	{\label{fig:us_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/us_acc_time_curve.png}}
  \caption{\small \textit{Left}: TPA performance per value of $C$ for both methods. \textit{Right}: CT performance per samples for both methods. 
  } \vspace{-10pt}
\label{fig:us_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:us_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/us_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance per value of $C$ of both methods for different rank values. \textit{Right}: CT performance per samples of both methods for different rank values.
  } \vspace{-10pt}
\label{fig:us_ranks_curve}  
\end{figure}


\begin{figure}%[t] 
  \centering
  	{\label{fig:bus_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/bus_acc_time_curve.png}}
  \caption{\small \textit{Left}: TPA performance per value of $C$ for both methods. \textit{Right}: CT performance per samples for both methods. 
  } \vspace{-10pt}
\label{fig:bus_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:bus_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/bus_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance per value of $C$ of both methods for different rank values. \textit{Right}: CT performance per samples of both methods for different rank values.
  } \vspace{-10pt}
\label{fig:bus_ranks_curve}  
\end{figure}

\subsection{Coverage Planning with Real-Time Map Prediction}
\subsubsection{Introduction to Experimental Methods}
We conduct coverage planning on the maze map as shown in Fig.~\ref{fig:tsp_results}-(a), which has a rank of 7. In this paper, we assume our vehicle for performing coverage planning is a point robot and no dynamics is considered. In Section.~\ref{sec:map_completion}, we have shown with a proper choice of $C$, the offline static map completion performance is outstanding and we also conclude there that a reference value for $C$ could be set to 2.0. However, in coverage planning, the observed entries are incrementally revealed since the robot needs to take time to traverse the area and only the places the robot has traversed could become observed entries in the matrix. To find a path for robot to perform the environmental monitoring, typical coverage planning methods used in real applications include: \textit{Lawn-Mower}~(LM), \textit{Global Random Sampling}~(GRS) and \textit{Traveling Salesman Problem}~(TSP).

LM: A simple but widely used classical coverage planning method. Given the size of the mapping area, a path with carefully designed interval is computed such that the whole area could be swept incrementally by the robot.

GRS: A global random sampling based method, in which at each action step, a set of points are randomly sampled in all unexplored areas and the closest one to the robot is selected as the local goal and a series of way-points are generated correspondingly. The robot only takes the first way-point for execution.

TSP: To follow the random uniform observation pattern in the LRMC model, we first uniformly sample a set of way points, then an existing TSP solver is used to find a shortest path connecting all the sampled way points. Note that being different to LM and GRS, TSP is a planning method that is compatible with our proposed LRMC model. The procedure of \textit{random uniform sampling way points} before performing TSP satisfies the assumption for the observation set $\Omega$ in LRMC while the number of way points is guided by Eq.~(\ref{eq:sampled_cond}) and a reference value for $C$ is discussed in Section.~\ref{sec:map_completion}. We will show in later experiments that because TSP based coverage planning is able to satisfy the assumptions in LRMC model, thus it outperforms other planning methods in terms of coverage convergence.

Before we start the experiment, we must determine the number of way points in TSP based planning. In a static environmental monitoring scenario, for example, in static sensor placement problem, the number of sampled observation points guided by Eq.~(\ref{eq:sampled_cond}) can be defined as:
\begin{equation}
    \label{eq:sample_num}
    N^{'}_{s} = \left \lfloor \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N^{'}_{s}$ represents the sensor positions number and $N$ is the number of observation entries within the sensor's local sensing range. Each sampled point will become a sampled block when sensor starts to run. Nevertheless, in the coverage planning scenario, the robot can take observations in between a pair of connected sampled way points and may introduce additional observations. This implies we may want to reduce the number of sampled way points as suggested by Eq.~(\ref{eq:sample_num}) and we do this by introducing a scale factor $\epsilon$ to Eq.~(\ref{eq:sample_num}):
\begin{equation}
    \label{eq:new_sample_num}
    N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor = \left \lfloor \epsilon \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N_{s}$ is the number of sampled way points in TSP planning and here we fix the value of $C$ as 2.0. Once the points are sampled using Eq.~(\ref{eq:new_sample_num}), a shortest path will be formed using a TSP solver and thereafter our robot could start the coverage mission by following the path. We name TSP planning with different $\epsilon$ values as: $TSP\_\epsilon$, where the $\epsilon$ is the scale factor in Eq.~(\ref{eq:new_sample_num}) and will be replaced with some specific values in experiments.

\subsubsection{Coverage Quality Analysis}
We compare the coverage convergence performance~(per action step) of \textit{LM}, \textit{GRS} and $TSP\_\epsilon$, where $\epsilon \in \left \{ 0.25,~0.5,~0.75 \right \}$, on the same underlying maze map~(as shown in Fig.~\ref{fig:tsp_results}-(a)). The results are shown in Fig.~\ref{fig:coverage}. 

\begin{figure*}%[h!]
  \centering
  \begin{subfigure}[b]{0.19\linewidth}
    \includegraphics[width=\linewidth]{figs/map_truth.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.39\linewidth}
    \includegraphics[width=\linewidth]{figs/coverage_half_0.5.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.39\linewidth}
    \includegraphics[width=\linewidth]{figs/coverage_0.5.png}
    \caption{}
  \end{subfigure}
  \caption{\small (a)~Ground-truth map for coverage planning. (b)~\textit{Left}: Real sensed map and \textit{Right}: predicted map at the middle of steps for TSP\_{0.5}. (c)~\textit{Left}: Real sensed map and \textit{Right}: predicted map at the ending step for TSP\_{0.5} }
  \label{fig:tsp_results}
\end{figure*}

\begin{table*}%[h]
\caption{Coverage performance comparison} %title of the table
\centering % centering table
\begin{tabular}{c rrrrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & 20\% & 40\% & 50\% & 60\% & 80\% & 90\% & 100\% \\
\hline % inserts single-line
LM & \vline & 153 / 69 & 310 / 141 & - / 176 & - / 212 & - / 285 & - / 320 &  - / 356~(99\%)\\ [1ex]% Entering row contents
GRS & \vline & 238 / 38 & - / 130 & - / 155 & - / 162 & - / 456 & - / 566 & - / -\\ [1ex]% [1ex] adds vertical space
TSP\_0.25 & \vline & 124 / 37 & - / 47 & - / 70 & - / \textbf{84} & - / \textbf{110} & - / \textbf{151} & - / - \\ [1ex]
TSP\_0.5 & \vline & 127 / 19 & - / 72 & - / 101 & - / 113 & - / 137 & - / 195 & - / \textbf{251}~(98\%)\\ [1ex]
TSP\_0.75 & \vline & 120  / \textbf{16} & 269 / \textbf{32} & - / \textbf{61} & - / 88 & - / 131 & - / 240 & - / \textbf{309} \\
\hline % inserts single-line
\end{tabular}
\label{tb:coverage_comparison}
\end{table*}

We first consider the coverage planning without real-time map prediction, and the results are shown in the left graph of Fig~\ref{fig:coverage}. We can see that due to the sensor limitations, none of the listed methods could perform a complete coverage planning without the functionality of map prediction. One may argue that we can perform map prediction~(or regression) on the incomplete map after the mission finishes. This off-line map prediction does work to help human obtain a finer-resolution feature map, but it does also have problems if we want to monitor the space online or the planning algorithm require an online updated fine-grain map to make decisions in real-time. We then consider the coverage planning with real-time map prediction, as shown in the right graph of Fig~\ref{fig:coverage}. With the aid of real-time map prediction, nearly all of the planning methods could obtain a complete~(almost $100\%$) feature map. In addition, the rate for coverage convergence is improved outstandingly for all of the listed coverage planning methods compared to themselves without real-time map prediction. We also claim that our proposed LRMC map prediction could be easily plugged with other planning methods that are not listed in this paper and facilitate their environmental monitoring performance.

According to the right graph of Fig~\ref{fig:coverage}, among all the coverage planning methods, TSP\_$\epsilon$ methods significantly outperform all the baseline methods in terms of coverage convergence, although TSP based method can reach different completeness level as the value of $\epsilon$ varies. Empirically a larger value of $\epsilon$ can lead to more sample points, a longer path~(and action step) from TSP, but as well as a better completeness~(i.e., TSP\_{0.75}). A proper choice of $\epsilon$ value can give us a satisfactory trade-off between completeness and required action steps. For example, if we have enough energy supply and pursuit a well completed feature map, we should select a big value of $\epsilon$, such as 0.75. On the other hand, we can have a moderate magnitude $\epsilon$, like 0.25 to achieve an acceptable coverage ratio~(i.e., 90\%), if we have limited energy or constrained allowed action steps. Even with extremely restricted number of action steps~(i.e., less than 200), with a proper $\epsilon$, our TSP based method~(i.e., TSP\_{0.25}, TSP\_{0.5}, and TSP\_{0.75}) can still achieve around $90\%$ coverage. The mapping results at the middle of steps and ending step for TSP\_{0.5} are shown in Fig.~\ref{fig:tsp_results}-(b) and Fig.~\ref{fig:tsp_results}-(c), respectively. From Fig.~\ref{fig:tsp_results}-(b), we can see that our proposed method could perform map interpolation and extrapolation simultaneously on-the-fly during the execution of environmental monitoring.

\begin{figure}[t] 
  \centering
%   \subfigure[]
  	{\label{fig:coverage}\includegraphics[width=\linewidth]{figs/coverage.png}}
  \caption{\small Coverage convergence per action step for different coverage planning methods \textit{Left}: without real-time map prediction and \textit{Right}: with real-time map prediction.
  } \vspace{-10pt}
\label{fig:coverage}  
\end{figure}

We also list the required number of action steps of all planning methods for different levels of completeness in Table~\ref{tb:coverage_comparison}. The format for the entries in Table~\ref{tb:coverage_comparison} is \textit{\# without real-time map prediction}~/~\textit{\# with real-time map prediction}. It is clear to see that the TSP\_$\epsilon$ methods can achieve remarkable reduction for required action steps at all listed completeness quantiles.










==> icra21/06_conclusions.tex <==
\section{CONCLUSIONS}
We consider the map prediction problem encountered in an urban building layout mapping scenario, where the sensor measurements are noisy and sparse. We first model the underlying feature map as a maze map, which is proven to possess low-rank and incoherent structures. Then we propose to use \textit{Low-Rank Matrix Completion}~(LRMC) to perform the map prediction on maze-like environments. Our extensive experiments validate that (1) The LRMC method can simultaneously perform map interpolation and extrapolation; (2) The LRMC method outperforms another state-of-the-art mapping method---Bayesian Hilbert Mapping~(BHM) in terms of mapping accuracy and computation time and could update the entire feature map in real-time; (3) With our proposed real-time map prediction method, the coverage convergence of commonly used coverage planning methods in environmental monitoring could be substantially improved. 

==> icra21/0_abstract.tex <==
\begin{abstract}
In many autonomous mapping tasks, the maps cannot be accurately constructed due to various reasons such as sparse, noisy, and partial sensor measurements.  
We propose a novel map prediction method built upon recent success of \textit{Low-Rank Matrix Completion}. The proposed map prediction is able to achieve both map interpolation and extrapolation on raw poor-quality maps with missing or noisy observations. 
We validate with extensive simulated experiments that the approach can achieve real-time computation for large maps, and the performance is superior to state-of-the-art map prediction approach --- Bayesian Hilbert Mapping in terms of mapping accuracy and computation time.
Then we demonstrate that with the proposed real-time map prediction framework, the coverage convergence rate~(per action step) for a set of representative coverage planning methods commonly used for environmental modeling and monitoring tasks can be significantly improved.

\end{abstract}

==> icra21/1_introduction.tex <==
\section{INTRODUCTION}
Mapping is a critical functionality for an autonomous robot that needs to perform tasks in an initially unknown environment where an underlying map is constructed with onboard sensors. 
However, this can be challenging if the sensor measurements are inaccurate or if the environment can only be partially measured (sensed), which are commonly seen in autonomous mapping scenarios. 
For instance, the point clouds obtained from low-end proximity sensors (e.g., LiDAR, IR, Sonar) might be extremely sparse especially in spacious environments. The point clouds might also contain many outliers (noisy points). In addition, oftentimes a mapping robot cannot visit every spot of the environment and the traversed areas may only partially cover the space with only some small sub-regions being measured. 
Given the sparse, noisy, and partial observations, it is desirable that a complete map can be efficiently predicted to well match the ground-truth environment, which is the objective of this paper. 

More formally, the map prediction aims to predict map structure based on already known regions and could be categorized into two classes: interpolation and extrapolation. Map interpolation means given some observations (measurement samples), we want to predict the values \textit{in between} the sampled places;
Map extrapolation means given some observation samples (or map structures), we want to predict the map values \textit{beyond} the sampled places. 

\begin{figure} \vspace{5pt}
  \centering
%   \subfigure[]
  	{\label{fig:real}\includegraphics[width=\linewidth]{figs/real_examples.png}}
  \caption{\small Urban and residential environments reveal strong structured patterns, such as \textit{Left}: road (or street) network and \textit{Right}: buildings layout. These environments containing linear dependent structures can be modeled as low-rank-matrix maps.} 
\label{fig:real}  
\end{figure}


In this paper, we propose to use Low-Rank Matrix Completion~(LRMC) to leverage the ill-conditioned map data to predict the whole map. LRMC exploits some special structures, such as low rank~(or linear dependency) and incoherence hidden in underlying map to perform the prediction. Two examples that possess special patterns in urban/residential environments are shown in Fig.~\ref{fig:real}.
We first illustrate how a structured environmental map satisfies important assumptions required by LRMC model. Then we qualitatively demonstrate with an urban road network map that our proposed LRMC method outperforms state-of-the-art map prediction~(or regression) method -- Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian} which is a Bayesian extension of Hilbert Mapping~(HM)~\cite{ramos2016hilbert}, where the map prediction is treated as a kernelized logistic regression problem. BHM eliminates crucial regularization parameter tunning in HM, and outputs continuous maps where the occupancy value of any arbitrary point could be queried.

We conduct exhaustive simulations on a set of maze-like complex maps and quantitatively analyze that our proposed LRMC method is superior to BHM on the maps with varying linear patterns and different rank values. 
Finally we combine the proposed real-time map prediction with representative coverage planning methods commonly used for environmental mapping and monitoring, and show that the mapping coverage convergence could be significantly improved with high mapping accuracy. 

We summarize our contributions as follows:
\begin{itemize}
    \item 
    This is the first time to examine and report that many complex urban/residential environments possess low-rank and incoherent structure, and to apply Low-Rank Matrix Completion for map prediction based on sparse, noisy, and partially observed maps.
    \item
    Our proposed Low-Rank Matrix Completion based map prediction outperforms state-of-the-art map prediction method---Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and is able to perform prediction in real-time.
    \item
    We perform extensive simulations and demonstrate the remarkable effectiveness of our proposed method  which allows representative coverage planning methods to achieve faster mapping coverage convergence rates.  %commonly used in environmental mapping   can be substantially improved.
\end{itemize}


==> icra21/2_related_work.tex <==
\section{RELATED WORK}

Map prediction has been studied in occupancy mapping problems.  
Prevalent methods include Occupancy Girds Mapping~(OGM)~\cite{elfes1989using}, Gaussian Process Occupancy Mapping~(GPOM)~\cite{o2012gaussian, wang2016fast}, Hilbert Mapping~(HM)~\cite{ramos2016hilbert} and Bayesian Hilbert Mapping~(BHM)~\cite{senanayake2017bayesian}. Specifically, OGM belongs to discrete mapping and all grids are independent with each other. To eliminate the requirement of pre-defining discrete grids and the independence assumption in OGM, GPOM is proposed and used in many applications~\cite{jadidi2014exploration, jadidi2015mutual}. GPOM naturally captures the neighbouring information thanks to kernelization, but being a non-parametric model, it has a computation complexity of $O(n^3)$, where $n$ is the number of sampled data points. Combining various advantages of GPOM, a faster and simpler parametric model---HM and its Bayesian version, BHM, is proposed later to eliminate the cubical time complexity in GPOM.

Map extrapolation 
attracts increasing attention in recent years and almost all the current methods for map extrapolation are based on deep neural networks~(DNNs)~\cite{caley2019deep, pronobis2017learning, katyal2018occupancy, shrestha2019learned, saroya2020online, katyal2019uncertainty}. However, DNNs based methods require huge amount of data for training and hence are still limited in general applications. In this paper, we propose to use Low-Rank Matrix Completion to perform the map prediction. 
Our proposed LRMC based method falls in between the {interpolation} and {extrapolation} methods. Specifically, the LRMC method can not only well interpolate map values, but at the same time can  extrapolate the map structure beyond the explored areas. 

In the past two decades, the Low-Rank Matrix Completion~(LRMC) problem has been well studied. The first theoretically guaranteed exact LRMC algorithm is proposed in~\cite{candes2009exact}, where any $n \times n$ incoherent matrices of rank $r$ are proven to be exactly recovered from $C n^{1.2}r\log n$ uniformly randomly sampled entries with high probability through solving a convex problem of nuclear norm minimization~(NNM). Subsequent works~\cite{candes2010power, chen2015incoherence, gross2011recovering, recht2011simpler} refine the provable completion results following the NNM based method. However, since all of the algorithms mentioned above are based on second order methods~\cite{liu2010interior}, they can become extremely expensive if the matrix dimension is large~\cite{cai2010singular}. Some first order based methods~\cite{cai2010singular, ji2009accelerated, mazumder2010spectral} are developed later. They solve the nuclear norm minimization problem in an iterative manner and rely on Singular Value Decomposition~(SVD) of matrices and are suited to large-scale matrix completion problems. In recent years, many other techniques are developed, such as coherent matrix completion~\cite{liu2017new, bhojanapalli2014universal, chen2014coherent}, non-linear matrix completion~\cite{eriksson2012high} and adaptive sampling~\cite{chen2015completing, eftekhari2018mc2}. {\color{black}A recent survey on LRMC could be found in \cite{nguyen2019low}.}
In this paper, we mainly employ the first order SVD based iterative method, such as~\cite{mazumder2010spectral} to solve the LRMC problem. {\color{black} The SVD based methods are able to achieve low prediction error and maintain a low time complexity if certain special problem structure is appropriately leveraged~\cite{mazumder2010spectral}.}


==> icra21/3_methodology.tex <==
\section{METHODOLOGY}
\label{sect:method}

\subsection{Problem Description}
Map prediction exhibits the same form as the matrix completion \cite{recht2009simpler} while a 2D map can be treated as a matrix. We propose to use LRMC as the map prediction method. LRMC is defined as completing a partially observed matrix $\tilde{\mathbf{M}}\in\mathbb{R}^{n_1\times n_2}$ whose part of entries are missing and the corresponding ground-truth matrix $\mathbf{M}$ has a low-rank and incoherent structures. Since the ground-truth rank is usually unknown, a typical way to complete $\tilde{\mathbf{M}}$ is to find a minimal rank matrix $\mathbf{X}^*$ that is consistent with $\tilde{\mathbf{M}}$ on the observed entries. A formal mathematical definition is:
\begin{equation}
    \label{eq:mc_1}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&rank(\mathbf{X})\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega,
    \end{aligned}
\end{equation}
where $\Omega \subset \left \{ 1, \cdots, n_1 \right \}\times \left \{ 1, \dots, n_2 \right \} $ is an index set of locations corresponding to the observed entries~($\left ( i, j \right )\in \Omega$ if $M_{ij}$ is observed). 

\subsection{Low-Rank and Incoherent Structures}
Two important assumptions for the underlying matrix $\mathbf{M}$ must be satisfied to guarantee the matrix completion results:
\begin{itemize}
    \item 
    $\mathbf{M}$ should be a low-rank matrix. A low-rank matrix implies its rank value is much smaller than its dimension and this structure enables the possibility to leverage linear dependencies among columns and/or rows of a matrix to predict missing entries~\cite{ongie2018tensor}. 
    \item
    $\mathbf{M}$ should be an incoherent matrix, which means the coherence of $\mathbf{M}$ is low. Suppose that a \textit{compact} SVD of a rank-r matrix $\mathbf{M}\in \mathbb{R}^{n_1\times n_2}$ is $\mathbf{M} = \mathbf{U}\Sigma\mathbf{V}^T$, where $\mathbf{U} \in \mathbb{R}^{n_1\times r}$ and $\mathbf{V}\in \mathbb{R}^{n_2\times r}$ are stacked left and right singular vectors of $\mathbf{M}$, while $\Sigma \in \mathbb{R}^{r\times r}$ is the diagonal matrix formed by a number of $r$ singular values of $\mathbf{M}$. The statistical leverage scores of $\mathbf{U}$ and $\mathbf{V}$ are defined by $\gamma_{U} = \underset{i\in \left \{ 1, \cdots, n_1 \right \}}{\text{max}}\left \| \mathbf{U}_{i,~:} \right \|^2_2$ and $\gamma_{V} = \underset{j\in \left \{ 1, \cdots, n_2 \right \}}{\text{max}}\left \| \mathbf{V}_{j,~ :} \right \|^2_2$, respectively, where $\mathbf{U}_{i,~:}$ and $\mathbf{V}_{j,~:}$ represent the $i^{th}$ and $j^{th}$ row of $\mathbf{U}$ and $\mathbf{V}$. Then the coherence of $\mathbf{M}$ is defined as:
    \begin{equation}
        \label{eq:coherence}
        \gamma_{M} = \max \left \{ \gamma_{U}, \gamma_{V} \right \}.
    \end{equation}
    The value of $\gamma_M$ is within $\left [ 0, 1 \right ]$ and an incoherent structure means the value of $\gamma_M$ is near 0. A small coherence value implies that the mass of values in the matrix will not concentrate on small portions, but spread out through the whole matrix.
\end{itemize}

Under the two conditions, the matrix $\tilde{\mathbf{M}}$ has been shown to be provably recoverable~\cite{candes2009exact}. Fig.~\ref{fig:mazes_1} and Table~\ref{tb:maze_prop} illustrate the trends of ranks and coherences of different structured environments which are similar to complex versions of either urban road networks or building layouts.
We can observe that the typical structured environments have ranks below 100, which are significantly smaller compared to the original matrix dimensions which could be multiple magnitudes higher (e.g., $10^4$ or above). 
The trend of ranks also reflects the complexity of the environment, and the higher the rank is, the more complex the environment is.
Along with the rank values, we also list the coherence values computed by using Eq.~(\ref{eq:coherence}).
Although the coherence increases proportionally to the rank, they all stay at a low level indicating high incoherence. 

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:mazes_1}\includegraphics[width=0.99\linewidth]{figs/mazes_with_ranks.png}}
  \caption{\small Maze environments with different ranks.
  } \vspace{-10pt}
\label{fig:mazes_1}  
\end{figure}

\begin{table}[h]

\caption{Matrix properties of maze environments} %title of the table
\centering % centering table
\begin{tabularx}{\linewidth}{ccccccc}%{c rrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & (a) & (b) & (c) & (d) & (e) & (f)\\
\hline % inserts single-line
Rank & 2 & 7 & 11 & 14 & 19 & 22\\ % Entering row contents
Coherence & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabularx}
\label{tb:maze_prop}
\end{table}


\subsection{Solving LRMC in Map Prediction}
\label{sect:static}

To solve the LRMC problem, 
the rank minimization problem in Eq.~(\ref{eq:mc_1}) is non-convex and NP-hard unfortunately, and hence of little practical use. An alternative way for Eq.~(\ref{eq:mc_1}) is to replace $rank(\mathbf{X})$ with $\left \| \mathbf{X} \right \|_*$, where $\left \| \mathbf{X} \right \|_*$ is the nuclear norm of $\mathbf{X}$, that is, the sum of sigular values of $\mathbf{X}$: $\left \| \mathbf{X} \right \|_* = \sum_{k=1}^{\min \left \{ n_1, n_2 \right \}}\sigma_k(\mathbf{X})$, where $\sigma_k(\mathbf{X})$ is the $k^{th}$ largest singular values of $\mathbf{X}$. The new formulation is:
\begin{equation}
    \label{eq:mc_2}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega.
    \end{aligned}
\end{equation}
The nuclear norm $\left \| \mathbf{X} \right \|_*$ is an effective convex relaxation to the rank objective and the optimization in Eq.~(\ref{eq:mc_2}) could be solved by semi-definite programming~\cite{laurent2014positive}.

Nevertheless, the optimizations in Eq.~(\ref{eq:mc_1}) and Eq.~(\ref{eq:mc_2}) aim to exactly recover the partially observed matrix, and this way was claimed as too rigid and may result in over-fitting~\cite{mazumder2010spectral}. A more robust way is to add a regularization parameter in Eq.~(\ref{eq:mc_2}):
\begin{equation}
    \label{eq:mc_3}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && \sum_{(i, j)\in \Omega}(X_{ij} - M_{ij})^2\leq \delta,
    \end{aligned}
\end{equation}
where $\delta \geq 0$ is a parameter regulating the training error tolerance. Equivalently Eq.~(\ref{eq:mc_3}) could be reformulated in a Lagrange form:
\begin{equation}
    \label{eq:mc_4}
    \begin{aligned}
        \mathbf{X}^* = \underset{\mathbf{X}}{\text{argmin}} \sum_{(i, j)\in \Omega} (X_{ij} - M_{ij})^2 + \lambda \left \|\mathbf{X} \right \|_{*},
    \end{aligned}
\end{equation}
where $\lambda$ is a regularization parameter controlling the nuclear norm. A SVD based iterative method proposed in~\cite{mazumder2010spectral} can be used to solve the Eq.~(\ref{eq:mc_4}).


\subsection{Mapping with Non-myopic Planner}
\label{sect:plan}

We are intrigued if the proposed map prediction can facilitate and improve existing environmental mapping and coverage methods. Popular planning paradigms include lawnmower mapping~\cite{li2019coverage, song2018varepsilon}, myopic (short-horizon) planning~\cite{khan2014greedy}, as well as non-myopic (long-horizon) planning~\cite{ kantaros2019asymptotically}. Lawnmower planning pursues complete spatial coverage, and myopic methods are oftentimes greedy schemes. The non-myopic approaches have been favored by many researchers for environmental mapping and monitoring~\cite{ma2016information, chen2019pareto}. Since non-myopic planners optimize paths over some horizon, we adopt and adapt the standard  \textit{Traveling Salesman Problem}~(TSP), which will be used in our evaluation in the experimental section. 

A TSP 
can be defined as that, given the positions of a collection of way points, what is the shortest possible path of reaching each way point only once and eventually returning to the starting point. 
To efficiently solve the TSP, we extend our recently developed adaptive \textit{k}-opt method~\cite{ma2016adaptive} which exploits and modifies the adaptive $k$-swap mechanism originally designed for multi-agent
task allocation. The core idea is to approximate the NP-hard problem with an opportunistic and localized tour improvement heuristic by taking account of tour
constraints adaptively and flexibly, so that real-time solution can be obtained with small sacrifice on solution accuracy. 

To determine the number of the way points for navigation guidance in TSP, previous work~\cite{candes2009exact} has theoretically proven that a partially observed low-rank matrix could be perfectly recovered if the number of sampled entries $m$ obeys:
\begin{equation}
    \label{eq:sampled_cond}
        m\geq Cn^{1.2}r\log n,
\end{equation}
where $C$ is a positive numerical coefficient, $n = \max\left \{ n_1, n_2 \right \}$, and $r$ is the rank of the underlying matrix $\mathbf{M}$~\cite{candes2009exact}. Based on Eq.~(\ref{eq:sampled_cond}),
the placements of way points
can be defined
as:
\begin{equation}
    \label{eq:sample_num}
    N^{'}_{s} = \left \lfloor \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N^{'}_{s}$ represents the number of way points and $N$ is the number of observed map samples within each way point's local sensing range. 
Note that, in coverage planning scenarios, the robot can take observations in between any pair of successive sampling way points and may introduce additional observations. This implies we may want to reduce the number of sampled way points, 
and we do this by using a scale factor $\epsilon$, so that $N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor$, 
where $N_{s}$ is the number of sampled way points in TSP planning. 
We name this TSP based planning with different $\epsilon$ values as $TSP\_\epsilon$. 
Once a number of $N_{s}$ points are sampled, a fast and  near-shortest path will be formed using the adaptive \textit{k}-opt TSP solver and thereafter our robot could start the coverage mission by following the path. 




==> icra21/4_experiments.tex <==
\section{EXPERIMENTS}

To validate the proposed framework, we perform extensive simulation evaluations with a variety of complex maps. 

\subsection{Experimental Setups and Metrics Design}

To account for the sensor limitations as in robotics applications, we use two measurement patterns, \textit{Noisy Observation}~(NO) and \textit{Partial Observation}~(PO), for constructing the $\Omega$. NO means the observations are imperfect due to random noises (e.g., due to factors of environments/weathers such as snows, or sensor hardware limitations such as sparse and noisy measurements); 
PO means missed or uncovered regions which are typical in environmental mapping and monitoring scenarios. 

To quantitatively compare the two methods,  we use two evaluation metrics, \textit{total prediction accuracy}~(TPA), and \textit{computational time}~(CT). TPA indicates the correct entry matches (including the observed entries) between the entire predicted map and the ground-truth map while CT measures the required time for map prediction computation. 
In addition, we also evaluate the \textit{mapping convergence rate} during the coverage planning.


\subsection{Demonstration with Road Network Mapping}
\begin{figure}
  \centering
%   \subfigure[]
  	{\label{fig:road_image}\includegraphics[width=\linewidth]{figs/road_image.png}}
  \caption{\small \textit{Left}: road network displays linear dependent structures.  \textit{Right}: The road network is extracted where 
  the dark color represents the road while others are off-road places.
  } 
\label{fig:road_image}  
\end{figure}

\begin{figure} %\vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_comparison}\includegraphics[width=\linewidth]{figs/road_comparison.png}}
  \caption{\small Comparison between LRMC and BHM under NO~(first row) and PO~(second row) patterns, respectively. (a)\&(e)~Ground-truth maps. (b)\&(f)~Partially observed maps for NO and PO patterns. The missing parts are indicated in green patches. (c)\&(g)~Predicted maps from LRMC model. (d)\&(h)~Predicted maps from BHM.
  } \vspace{-10pt}
\label{fig:road_comparison}  
\end{figure}



We first demonstrate that our proposed LRMC method is able to perform map interpolation and extrapolation on a road network map extracted from an  urban environmental map, as shown in Fig.~\ref{fig:road_image}. 
The road surface can be detected by proximity sensors such as IR. We assume the robot is an aerial vehicle so that it can spot regions locally below it. 

The comparison of the two mapping methods on the urban road map under NO and PO patterns can be seen in Fig.~\ref{fig:road_comparison}. With NO pattern, both methods can generally predict the road network pattern~(topology), although BHM is more sensitive to the noises and thus fails to capture the exact road shape. On the other hand, with PO pattern, LRMC significantly outperforms BHM in the presence of multiple missing patches. 
Different from NO pattern, PO requires that the map prediction not only has interpolation capability, but also can perform slight extrapolation to reason the map structure within missing patches. 
LRMC leverages the linear dependency among the rows/columns of the map matrix and is able to predict the structure even multiple missing patches occur. In contrast, although BHM can capture local neighbouring spatial relationship by using kernelization, it is unable to capture the linear dependency brought by the low-rank structure, and thus performs worse than LRMC. 

\subsection{Quantitative Comparison between LRMC and BHM}

We first generate 20 differing complex maze-like layouts/environments by using the Daedalus tool~\cite{daedalus}, and consider the TPA and CT statistical comparisons under NO and PO patterns for different values of $C$. 
The results are shown in Fig.~\ref{fig:us_acc_time_curve} and Fig.~\ref{fig:bus_acc_time_curve}. 
The trend of TPA and CT in different rank-valued maps %with different $C$ 
are shown in Fig.~\ref{fig:us_ranks_curve} for NO and Fig.~\ref{fig:bus_ranks_curve} for PO, respectively.

We first analyze the results for NO pattern. In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, it can be observed that 
LRMC could achieve a higher accuracy level. 
From Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we want to determine a proper scale of the coefficient $C$. We can think the coefficient $C$ is actually reflecting the number of observed map samples according to Eq.~(\ref{eq:sampled_cond}). 
In Fig.~\ref{fig:us_acc_time_curve}-\textit{Left}, we can see that TPA could reach a high level and stay stable when $C\geq 1.5$.
We then compare the CT performance as shown in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}. The result clearly distinguishes the two methods. The required computation time for LRMC is much lower than that of BHM. Given the size of the entire map~(matrix), the computational complexity of the LRMC algorithm~(SoftImpute~\cite{mazumder2010spectral}) we use is $O((m+n)r^2)$, where $m$ and $n$ are the dimensions and $r$ is the rank of the underlying ground-truth matrix. This means the LRMC model has a constant time complexity regardless of the number of observations. BHM is a logistic regression based method and has linear time complexity in terms of the number of observations. 

\begin{figure} 
  \centering
  	{\label{fig:us_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/us_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under NO pattern from 20 different mazes~(with different linear dependencies but the same rank). 
  } \vspace{-10pt}
\label{fig:us_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:us_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/us_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under NO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:us_ranks_curve}  
\end{figure}


\begin{figure}%[t] 
  \centering
  	{\label{fig:bus_acc_time_curve}\includegraphics[width=0.99\linewidth]{figs/bus_acc_time_curve.png}}
  \caption{\small \textit{Left}: Statistical TPA performance and \textit{Right}: CT performance per value of $C$ for LRMC and BHM under PO pattern from 20 different mazes~(with different linear dependencies but the same rank).  
  } \vspace{-10pt}
\label{fig:bus_acc_time_curve}  
\end{figure}

\begin{figure}%[t]
  \centering
  	{\label{fig:bus_ranks_curve}\includegraphics[width=0.99\linewidth]{figs/bus_ranks_curve.png}}
  \caption{\small \textit{Left}: TPA performance and \textit{Right}: CT performance per value of $C$ of both methods under PO pattern on different maps with varying values of rank.
  } \vspace{-10pt}
\label{fig:bus_ranks_curve}  
\end{figure}

Note however, from Fig.~\ref{fig:us_acc_time_curve}-\textit{Right} we can see that the LRMC model has a better CT performance than constant time! The reason for this is the LRMC algorithm we use relies on SVD of the matrix. SVD is the most efficient for  dense matrices but not that efficient for sparse ones. In our case,   at first the number of observations can be small so the input matrix is a sparse one. 
The runtime benefit will actually  increase with more observations received, which is a significant feature for real-time robot mapping applications.  

In Fig.~\ref{fig:us_ranks_curve}, we compare the TPA and CT for environments with different ranks. It is clear to see in Fig.~\ref{fig:us_ranks_curve}-\textit{Left} that when the environment becomes more complex~(as the rank value increases), the accuracy of BHM decreases while LRMC maintains the same high-level prediction~(almost $100\%$). From the first row of Fig.~\ref{fig:road_comparison}, we can find BHM generally performs well but many minor discrepancies can be found along the road edges.  When the environment becomes complex, the number of edges increases and thus the minor errors accumulate and this results in the increase of the total map prediction error. The time performances~(Fig.~\ref{fig:us_ranks_curve}-\textit{Right}) of the two methods for different rank-valued maps show the same trend as in Fig.~\ref{fig:us_acc_time_curve}-\textit{Right}.

We then consider the results under PO pattern. Similar to what we have in the NO pattern, the TPA and CT results are shown in Fig.~\ref{fig:bus_acc_time_curve} and Fig.~\ref{fig:bus_ranks_curve}, respectively. The comparison results follow similar trends to the NO pattern. 

\subsection{Coverage Planning with Real-Time Map Prediction}

We investigate if the proposed map prediction can facilitate and improve existing environmental mapping and coverage planning methods. 
Our evaluations are based on three most prevalent strategies. 
The first planning method is the lawnmower (LM) planning: a simple but the most widely used coverage planning method in environmental surveying and monitoring.  Specifically, the traversal patterns and resolutions are pre-determined such that the whole area could be swept incrementally by the robot.
The second planning is the myopic planning (MP) which is typically based on greedy choices (or best-first actions). Here at each action step, a set of points are randomly sampled in all unexplored areas and the closest one to the robot is selected as the local goal. 
The third planning is the non-myopic customized $TSP\_\epsilon$ as described in Section~\ref{sect:plan}, 
where $\epsilon \in \left \{ 0.25,~0.5,~0.75 \right \}$.

\begin{figure*} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:road_tsp}\includegraphics[width=0.9\linewidth]{figs/road_tsp.png}}
  \caption{\small Environmental mapping of an urban road map using TSP\_{0.5}. The path is calculated by using an adaptive \textit{k}-opt TSP planner.
  In each of (a), (b), (c) and (d),  the \textit{Left} figure denotes the observed map while \textit{Right} is the predicted map using LRMC model, respectively. 
  } \vspace{-10pt}
\label{fig:road_tsp}  
\end{figure*}
% \begin{figure*} %\vspace{-3pt}
%   \centering
% %   \subfigure[]
%   	{\label{fig:terrain_tsp}\includegraphics[width=0.95\linewidth]{figs/terrain_tsp.png}}
%   \caption{\small {\color{blue} Environmental mapping of an terrain map using TSP\_{0.5}. The path~(yellow lines) is calculated by using an adaptive \textit{k}-opt TSP planner.
%   In each of (a), (b), (c) and (d),  the \textit{Left} figure denotes the observed map while \textit{Right} is the predicted map using LRMC model, respectively. }
%   } \vspace{-10pt}
% \label{fig:terrain_tsp}  
% \end{figure*}

\begin{figure}[t] 
  \centering
%   \subfigure[]
  	{\label{fig:coverage}\includegraphics[width=\linewidth]{figs/coverage.png}}
  \caption{\small Coverage convergence per action step for different coverage planning methods \textit{Left}: without real-time map prediction and \textit{Right}: with real-time map prediction.
  } \vspace{-10pt}
\label{fig:coverage}  
\end{figure}

The mapping process with non-myopic planning on the urban road network map is demonstrated in Fig.~\ref{fig:road_tsp}, where the real observed (sensed) map and corresponding predicted map from LRMC at four different action steps are presented. The results are consistent with that shown in Fig.~\ref{fig:road_comparison}.

To statistically evaluate the methods, we first consider the coverage planning with only raw observations but no map prediction. (As mentioned earlier, real-time predicted complete maps might not be available due to expensive computation cost in large environments.) The results are shown in Fig.~\ref{fig:coverage}-\textit{Left}, in which none of the listed methods could complete the map coverage within the given number of steps.
This also implies the necessity of real-time map prediction, 
and the results with map prediction are shown in Fig.~\ref{fig:coverage}-\textit{Right}. 
We can see that, 
within the same or less number of steps, nearly all of the planning methods could obtain a complete~(almost $100\%$) mapping coverage with real-time map prediction. 
In addition, the rate for coverage convergence is also remarkably improved for all of the listed coverage planning methods.

According to Fig.~\ref{fig:coverage}-\textit{Right}, among all the coverage planning methods, TSP\_$\epsilon$ methods significantly outperform other methods in terms of coverage convergence, although TSP based method can reach different completeness level as the value of $\epsilon$ varies. 
Empirically a larger value of $\epsilon$ can lead to more observations, a longer path~(and action steps), but also a better level of completeness (i.e., TSP\_{0.75}). A proper choice of $\epsilon$ value can give us a satisfactory trade-off between completeness and required action steps. 
Even with extremely restricted number of action steps~(i.e., less than 200), with a proper $\epsilon$, the TSP based methods can still achieve around $90\%$ coverage. The mapping results at different action steps by TSP\_{0.5} are shown in Fig.~\ref{fig:road_tsp}-(a), (b), (c) and (d), where we can see that our proposed method is able to perform map interpolation and extrapolation simultaneously on the fly during the execution of environmental mapping.

We also list the required number of action steps of all planning methods for different levels of completeness in Table~\ref{tb:coverage_comparison}. It is clear to see that with the proposed real-time LRMC map prediction all coverage planning methods can obtain a substantial improvement of coverage quality, and the required action steps at all listed completeness quantiles are remarkably reduced compared to the results without real-time map prediction.

\begin{table}\vspace{2pt}%[h]
\caption{\small Required number of action steps for varying levels of coverage completeness for different methods. The format for the entries indicates \textit{\# without real-time map prediction}~/~\textit{\# with real-time map prediction}, where `-' means the corresponding method fails to finish the respective completeness level.} %title of the table
\centering % centering table
{%\footnotesize
\begin{tabularx}{0.85\linewidth}{ccccc}%{c rrrrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
   & 20\% & 50\%  & 90\% & 100\% \\[0.5ex]
\hline % inserts single-line
LM  & 153 / 69 & - / 176 & - / 320 &  - / 356~(99\%)\\ [1ex]% Entering row contents
MP & 238 / 38 & - / 155 & - / 566 & - / -\\ [1ex]% [1ex] adds vertical space
TSP\_0.25  & 124 / 37 & - / 70 & - / \textbf{151} & - / - \\ [1ex]
TSP\_0.5  & 127 / 19 & - / 101 & - / 195 & - / \textbf{251}~(98\%)\\ [1ex]
TSP\_0.75  & 120  / \textbf{16} & - / \textbf{61} &- / 240 & - / \textbf{309} \\
\hline % inserts single-line
\end{tabularx}
}
\label{tb:coverage_comparison} \vspace{-10pt}
\end{table}










==> icra21/5_conclusions.tex <==
\section{CONCLUSIONS}
We consider the map prediction problem where the measurements are noisy, sparse and partially observed. We first show that many maps possess low-rank and incoherent structures. Then we propose to use LRMC to perform the map prediction. Our extensive experiments validate that the LRMC method can effectively perform map prediction (interpolation and extrapolation), and the LRMC method outperforms  state-of-the-art Bayesian Hilbert Mapping in terms of mapping accuracy and computation time and could update the entire map in real-time. Lastly we show that the proposed real-time map prediction method can be easily combined with popular coverage planning methods and can significantly improve their coverage convergence rates.

==> old/0_abstract.tex <==
\begin{abstract}

Coverage planning may end up with a partially revealed feature map if only single robot is available for operation and given energy supplies or the allowed action steps are quite limited. In this paper, with an assumption that the underlying feature map exhibits some special structures~(i.e., low-rank and incoherent structures), we propose a map predictive coverage planning method building upon the theory of \textit{Low-Rank Matrix Completion}. The proposed map prediction avoids the massive data for training compared with existing widely used map prediction methods, i.e., deep neural network based map predictions and is computationally cheap, and thus could be used for coverage planning in real-time. We have validated our approach via extensive simulated experiments, and the evaluations reveal that compared to other coverage planning techniques, not only our solution be able to predict the partial feature map, but also can achieve significantly faster coverage convergence~(per action step), even with severely degraded local sensing quality.

\end{abstract}

==> old/1_introduction.tex <==
\section{INTRODUCTION}
One critical task for autonomous vehicles is coverage planning, which aims to cover/monitor a certain area of interest to obtain a feature map~(e.g., terrain map, building layout map, and chemical concentration map) by leveraging the flexible mobility of the robotic platform and the sensing capability of the sensors equipped on the vehicle. There have been intensive applications of coverage planning, including floor cleaning~\cite{oh2004complete, palacin2004building}, agriculture~\cite{hameed2013optimized, zhou2014agricultural, jin2010optimal}, structure inspection~\cite{englot2012sampling, ellefsen2017multiobjective}, terrain reconstruction~\cite{krotkov1994terrain, torres2016coverage}, oil spills cleaning~\cite{song2013adaptive}, and environmental monitoring~\cite{he2019autonomous}. Aerial vehicles become particularly popular for performing coverage planning missions due to its high agility, low cost and unique down-facing field of view from the air. However, aerial robots notoriously suffer from the limited on-board resources (e.g, power supply), which may result in a partial coverage for a single aerial vehicle if the region to be explored is relatively large. The vast majority of prior works assume the robot is energy-free when considering the feature map coverage problem. Only recent few works consider energy consumption limitations~\cite{di2016coverage, modares2017ub, cabreira2018energy} and consequent partial coverage~\cite{ellefsen2017multiobjective, papachristos2016distributed, jensen2020near}. Although~\cite{di2016coverage, modares2017ub, cabreira2018energy} consider to optimize coverage path with respect to power assumption, most of them still require the robot has enough energy to achieve resolution-complete coverage. Given limited power/flight time/path length, while \cite{di2016coverage, modares2017ub, cabreira2018energy} optimize the path to achieve a trade-off between their own limitations and coverage, they end their jobs with an incomplete feature map and fail to mention how to leverage the partially revealed information to predict the whole map. In this paper, we propose to use Low-Rank Matrix Completion~(LRMC) to leverage the partially observed map information to predict the whole feature map provided that we are dealing with a scenario where a single aerial vehicle is assigned to perform an urban building layout monitoring task~(where we assume no trees or other objects occluding the buildings) and the given power might be only enough to conduct a partial coverage planning. We carefully illustrate how urban environment terrain monitoring task fits into the LRMC model and demonstrate that partially revealed information can still provide sufficient clues to predict the uncovered regions if the underlying feature map possesses some intrinsic structure(e.g., low-rank and incoherent structures) in intensive experiments with two local sensing modes: \textit{perfect local sensing} and \textit{degraded local sensing}.

We summarize our contributions as follows:
\begin{itemize}
    \item 
    We are the first to examine and illustrate that maze-like environments possess low-rank and incoherent structure.
    \item
    We are the first to apply Low-Rank Matrix Completion to predict the partially observed maze environments.
    \item
    We are the first to combine Low-Rank Matrix Completion with TSP to significantly enhance the energy-constrained coverage planning.
    \item
    We provide intensive simulated experiments and demonstrate the outstanding effectiveness of our proposed method compared with other alternate coverage planning solutions. We emphasize that our method is particularly suited with real scenarios, where local sensed map may contain many missing parts due to the sensor limitations.
\end{itemize}


==> old/2_related_work.tex <==
\section{RELATED WORK}
Our work on map prediction based coverage planning is related to classical coverage planning and map structure prediction. In classical coverage planning, the most efforts are made on development of planning algorithms, while quite few works consider the potential benefits from combining map prediction. However, most of the current map prediction techniques rely on deep learning~\cite{caley2019deep, pronobis2017learning, katyal2018occupancy, shrestha2019learned, saroya2020online}, requiring extremely large datasets to achieve a reasonable results in certain types of environments. We want to avoid the data-demanding deep learning based methods and leverage Low-Rank Matrix Completion to enable the functionality of map prediction. We survey related efforts in those directions. 

\textbf{Classic Coverage Planning.} Classic approaches for coverage planning mainly focus on planning algorithms and seek to achieve a resolution-complete coverage. Many factors are considered in planning to improve the coverage performance, such as non-holonomic mobility constraints~\cite{kan2020online}, submodularity-based multi-agent network~\cite{sun2017submodularity}, and hexagonal cell decomposition~\cite{paull2012sensor}. Most of prior works~\cite{oh2004complete}-\cite{he2019autonomous},~\cite{kan2020online}-\cite{paull2012sensor} assume that the robot has enough power to complete the mission. Some recent works~\cite{ellefsen2017multiobjective},~\cite{di2016coverage}-\cite{cabreira2018energy}, \cite{papachristos2016distributed}-\cite{jensen2020near},~\cite{li2019coverage} start to consider the coverage planning under the energy constraints. While they take the power constraints into consideration, they lack solutions for the situations where the mission ends up with an incomplete feature map. Note that none of all prior coverage planning works consider to use feature map prediction to enhance the coverage planning.

\textbf{Map Prediction.} Map prediction aims to predict map structure based on already revealed regions. Most of the current map structure predictions base their methods on deep neural networks (DNNs), which require massive training data. In~\cite{caley2019deep}, a database of building blueprints is used to train a DNN to predict exit locations of buildings. A single and universal model of the robot's spatial environment is learned by combining Sum-Product Networks~(SPNs) and deep learning in~\cite{pronobis2017learning}. An occupancy map representations of sensor data is predicted for future robot motions using DNNs in~\cite{katyal2018occupancy}. A state-of-the-art generative DNN is used in~\cite{shrestha2019learned} to predict unknown regions of a partially explored map and then the prediction is used to enhance the exploration in an information-theoretic manner. Some special map structure, such as topological maps that resemble the sparse subterranean tunnel networks, are predicted using a convolutional neural network~(CNN) in~\cite{saroya2020online}. 

\textbf{Low-Rank Matrix Completion.} In the past two decades, the Low-Rank Matrix Completion~(LRMC) problem has been widely studied. The first theoretically guaranteed exact LRMC algorithm is proposed in~\cite{candes2009exact}, where any $n \times n$ incoherent matrices of rank r are proven to be exactly recovered from $C n^{1.2}r\log n$ uniformly randomly sampled entries with high probability through solving a convex problem of nuclear norm minimization~(NNM). Subsequent works~\cite{candes2010power, chen2015incoherence, gross2011recovering, recht2011simpler} refine the provable completion results following the NNM based method. However, since all of the algorithms mentioned above are based on second order methods~\cite{liu2010interior}, they can become extremely expensive if the matrix dimension is large~\cite{cai2010singular}. Some first order based methods~\cite{cai2010singular, ji2009accelerated, mazumder2010spectral} are developed to overcome the limitations of the second-order based methods. They solve the nuclear norm minimization problem in an iterative manner and rely on Singular Value Decomposition~(SVD) of matrices and are suited to large-scale matrix completion problems.

==> old/3_preliminaries.tex <==
\section{PRELIMINARIES}

\subsection{Low-Rank Matrix Completion}
\textit{Low-Rank Matrix Completion} is defined as completing a partially observed matrix $\tilde{\mathbf{M}}\in\mathbb{R}^{n_1\times n_2}$ whose part of entries are missing and the corresponding ground-truth matrix $\mathbf{M}$ has a low-rank structure, which indicates $rank(\mathbf{M})\ll \min \left \{ n_1, n_2 \right \}$. Since the ground-truth rank is unknown at most times, a typical way to complete $\tilde{\mathbf{M}}$ is to find a minimal rank matrix $\mathbf{X}^*$ that is consistent with $\tilde{\mathbf{M}}$ on the observed entries. A formal mathematical definition is:
\begin{equation}
    \label{eq:mc_1}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&rank(\mathbf{X})\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega,
    \end{aligned}
\end{equation}
where $\Omega \subset \left \{ 1, \cdots, n_1 \right \}\times \left \{ 1, \dots, n_2 \right \} $ is an index set of locations corresponding to the observed entries~($\left ( i, j \right )\in \Omega$ if $M_{ij}$ is observed). Unfortunately, the rank minimization problem in Eq.~(\ref{eq:mc_1}) is non-convex and NP-hard, and hence of little of practical use. An alternative way for Eq.~(\ref{eq:mc_1}) is to replace $rank(\mathbf{X})$ with $\left \| \mathbf{X} \right \|_*$, where $\left \| \mathbf{X} \right \|_*$ is the nuclear norm of $\mathbf{X}$, that is, the sum of sigular values of $\mathbf{X}$: $\left \| \mathbf{X} \right \|_* = \sum_{k=1}^{\min \left \{ n_1, n_2 \right \}}\sigma_k(\mathbf{X})$, where $\sigma_k(\mathbf{X})$ is the $k^{th}$ largest singular values of $\mathbf{X}$. The new formulation is:
\begin{equation}
    \label{eq:mc_2}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && X_{ij} = M_{ij},~~\left ( i, j \right )\in \Omega.
    \end{aligned}
\end{equation}
The nuclear norm $\left \| \mathbf{X} \right \|_*$ is an effective convex relaxation to the rank objective and the optimization in Eq.~(\ref{eq:mc_2}) could be solved in semidefinite programming.

However, the optimizations in Eq.~(\ref{eq:mc_1}) and Eq.~(\ref{eq:mc_2}) aim to exactly recover the partially observed matrix, and this way was claimed as too rigid and may result in over-fitting~\cite{mazumder2010spectral}. A more robust way is to add a regularization parameter in Eq.~(\ref{eq:mc_2}):
\begin{equation}
    \label{eq:mc_3}
    \begin{aligned}
        \mathbf{X}^* = ~&\underset{\mathbf{X}}{\text{argmin}} 
               &&\left \| \mathbf{X} \right \|_*\\
               &\text{subject to}
               && \sum_{(i, j)\in \Omega}(X_{ij} - M_{ij})^2\leq \delta,
    \end{aligned}
\end{equation}
where $\delta \geq 0$ is a parameter regulating the training error tolerance. Equivalently Eq.~(\ref{eq:mc_3}) could be reformulated in a Lagrange form:
\begin{equation}
    \label{eq:mc_4}
    \begin{aligned}
        \mathbf{X}^* = \underset{\mathbf{X}}{\text{argmin}} \sum_{(i, j)\in \Omega} (X_{ij} - M_{ij})^2 + \lambda \left \|\mathbf{X} \right \|_{*},
    \end{aligned}
\end{equation}
where $\lambda$ is a regularization parameter controlling the nuclear norm.
\subsection{Assumptions for Completion Guarantee}
Three important assumptions for the underlying matrix $\mathbf{M}$ and the observation set $\Omega$ must be satisfied to guarantee the matrix completion results according to~\cite{candes2009exact}:
\begin{itemize}
    \item 
    $\mathbf{M}$ should be a low-rank matrix. A low-rank matrix implies its rank value is much smaller than its dimension and this structure enables the possibility to leverage linear dependencies among columns and/or rows of a matrix to impute missing entries~\cite{ongie2018tensor}. 
    \item
    $\mathbf{M}$ should be an incoherent matrix, which means the coherence of $\mathbf{M}$ is low. Suppose that a \textit{compact} SVD of a rank-r matrix $\mathbf{M}\in \mathbb{R}^{n_1\times n_2}$ is $\mathbf{M} = \mathbf{U}\Sigma\mathbf{V}^T$, where $\mathbf{U} \in \mathbb{R}^{n_1\times r}$ and $\mathbf{V}\in \mathbb{R}^{n_2\times r}$ are stacked left and right singular vectors of $\mathbf{M}$, while $\Sigma \in \mathbb{R}^{r\times r}$ is the diagonal matrix formed by the $r$ singular values of $\mathbf{M}$. The statistical leverage scores of $\mathbf{U}$ and $\mathbf{V}$ are defined by $\gamma_{U} = \underset{i\in \left \{ 1, \cdots, n_1 \right \}}{\text{max}}\left \| \mathbf{U}_{i,~:} \right \|^2_2$ and $\gamma_{V} = \underset{j\in \left \{ 1, \cdots, n_2 \right \}}{\text{max}}\left \| \mathbf{V}_{j,~ :} \right \|^2_2$, respectively, where $\mathbf{U}_{i,~:}$ and $\mathbf{V}_{j,~:}$ represent the $i^{th}$ and $j^{th}$ row of $\mathbf{U}$ and $\mathbf{V}$. Then the coherence of $\mathbf{M}$ is defined as:
    \begin{equation}
        \label{eq:coherence}
        \gamma_{M} = \max \left \{ \gamma_{U}, \gamma_{V} \right \}.
    \end{equation}
    \item
    The observation set $\Omega$ should be randomly uniformly sampled and the number of the sampled entries $m$ should obey: 
    \begin{equation}
        \label{eq:sampled_cond}
            m\geq Cn^{1.2}r\log n,
    \end{equation}
    where $C$ is some positive numerical coefficient, $n = \max\left \{ n_1, n_2 \right \}$, and $r$ is the rank of the underlying matrix $\mathbf{M}$~\cite{candes2009exact}.
\end{itemize}




==> old/4_map_completion.tex <==
\section{MAP COMPLETION}
\label{sec:map_completion}

\begin{table*}%[h]
\caption{Matric properties of maze environments} %title of the table
\centering % centering table
\begin{tabular}{c rrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & (a) & (b) & (c) & (d) & (e) & (f)\\
\hline % inserts single-line
Rank & \vline & 2 & 7 & 11 & 15 & 19 & 23\\ % Entering row contents
Coherence & \vline & 0.0200 & 0.0400 & 0.0625 & 0.0833 & 0.1000 & 0.1250\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabular}
\label{tb:maze_prop}
\end{table*}

Map completion exhibits the same form as the matrix completion if the map is represented in a matrix. Typical forms of map encountered in coverage planning include occupancy map, elevation map~(terrain map), and certain interested value 2D distribution map~(e.g., temperature distribution, $CO_2$ distribution, etc.). A common property of those maps are that the values of interest are represented with real numbers that distribute in a 2D plane, for instance, occupancy values in occupancy maps; height values in elevation maps. If the values are discretely distributed in a 2D plane, then the map will become a matrix. In this paper, we call those maps as feature maps and address the prediction of a partially observed terrain map of urban environments, in which the places identified~(by an aerial vehicle from the air) as having buildings are treated as featured spaces, while other places as non-featured spaces. Following the definition of binary occupancy maps, we indicate the featured spaces as 1 while non-featured spaces as 0 such that the urban terrain map could be modeled as a maze map. In this section we show that a maze-like feature map satisfies the assumptions of the LRMC model and how LRMC model performs the prediction given a partially revealed maze map.

\begin{figure} \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:mazes_1}\includegraphics[width=0.9\linewidth]{figs/mazes_with_ranks.png}}
  \caption{\small Maze environments with different ranks. The value of 1.0 represents the featured space while 0.0 is the non-featured space.
  } \vspace{-10pt}
\label{fig:mazes_1}  
\end{figure}

\begin{figure}[t] \vspace{-3pt}
  \centering
%   \subfigure[]
  	{\label{fig:demo}\includegraphics[width=\linewidth]{figs/demo.png}}
  \caption{\small First row: Map completion with \textit{perfect local sensing}. (a)~Ground-truth maze map. (b)~Partially observed map. The missing parts are indicated with white blocks. (c)~The predicted map using LRMC model. Second row: Map completion with \textit{degraded local sensing}. The colors have the same meaning with the first row.
  } \vspace{-10pt}
\label{fig:demo}  
\end{figure}

Different maze maps with varying ranks are generated by Daedalus\footnote{\url{http://www.astrolog.org/labyrnth/daedalus.htm}} and are shown in Fig~\ref{fig:mazes_1}. Each map has a dimension of $20m \times 20m$ with a resolution of $0.1m$, which results in a matrix with dimension of $200\times 200$. The rank values are listed in Table~\ref{tb:maze_prop}. It is easy to observe that the value of rank basically reflects the complexity of the matrix. The higher the rank is, the more complex the environment is. A typical urban terrain (or building layout) map would be similar to the maze with rank of 11 (as shown in Fig.~\ref{fig:mazes_1}-(c)), which is also the rank parameter we adopt in this paper. Compared with the dimension of 200, 11 is a much smaller value and therefore enables the corresponding matrix to be called as a low-rank matrix. Even the maze environment becomes super complex, such as the one shown in Fig.~\ref{fig:mazes_1}-(f), the rank value is still relatively small compared with the matrix dimension. Along with the rank values, we also list the coherence value for each maze matrix using the Eq.~(\ref{eq:coherence}). Although the coherence increases proportionally to the rank, they all stay at a low-level where we can be convinced they all are incoherent. Hence we can conclude that maze environments generally possess the low-rank and low-coherence properties required by the LRMC model. 

The sensors used in coverage planning are usually interfered with exogenous factors~(such as wind disturbance, magnetic field, light conditions, etc.) and endogenous factors~(such as manufacturing limitations, installation error, etc.). Consequently, the raw measurements from sensors could be noisy and in many cases be sparse. In this section, we demonstrate the proposed LRMC based algorithm is robust to the degraded sensing measurements by considering two modes of local sensing: \textit{perfect local sensing}~(PLS) mode and \textit{degraded local sensing}~(DLS) mode when performing coverage tasks. The PLS mode assumes the local sensed map is in an ideal condition and the DLS mode assumes there always be some random parts are missed for each local sensory measurement. Throughout this paper, we adopt the  SoftImpute~\cite{mazumder2010spectral} for implementing the LRMC model and an example for map completion on a partially observed maze map with two local sense modes is shown in Fig.~\ref{fig:demo}. 

In this example, we randomly select near-half observations and apply the LRMC model to the partial matrix. We use two evaluation metrics here: \textit{pure prediction accuracy}~(PPA) and \textit{total prediction accuracy}~(TPA). The PPA represents the correct prediction on purely missing parts while TPA indicates the correct entry matches~(including the already observed parts) between the entire predicted maze and the ground-truth maze. TPA reflects the general completeness whereas PPA shows the pure prediction performance of the LRMC model on unexplored places. 
%the prediction performance by simultaneously considering the LRMC model and the already observed entries whereas PPA shows the pure prediction performance by only the LRMC model. 
The PPA and TPA results for two sensing modes are shown in Table~\ref{tb:exam_stat}. It is clear that even with less than half of revealed/observed entries, the LRMC model could achieve more than (or almost) $90\%$ correct predictions.



\begin{table}%[h]
\caption{Statistics for Fig.~\ref{fig:demo}} %title of the table
\centering % centering table
\begin{tabular}{c rrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & PLS & DLS\\
\hline % inserts single-line
Revealed percentage & \vline & 0.5132 & 0.4625\\ % Entering row contents
PPA & \vline & 0.8914 & 0.9326\\ % [1ex] adds vertical space
TPA & \vline & 0.9417 & 0.9638\\
\hline % inserts single-line
\end{tabular}
\label{tb:exam_stat}
\end{table}

Previous works have theoretically proven a partially observed low-rank matrix could be perfectly recovered if the number of sampled entries $m$ obeys the Eq.~(\ref{eq:sampled_cond})~\cite{candes2009exact}. Although the number of observation samples are theoretically lower bounded, it is still difficult to determine the exact value of the $m$ due to the existence of $C$. To determine a proper scale of the coefficient $C$, we generate 20 maze environments with the same rank of 11 and apply the LRMC model to different partially observed mazes and unveil the relationship between the coefficient $C$ and PPA/TPA. For each value of $C$ we compute a mean and standard deviation for TPA and PPA, respectively. The relation is shown in Fig.~\ref{fig:num_curves}.

We can think the coefficient $C$ is actually reflecting the number of observed entries according to Eq.~(\ref{eq:sampled_cond}). The higher the coefficient is, the more the observations are and the better the prediction is. From Fig.~\ref{fig:num_curves}, we can see that for PLS mode, the mean of both accuracies could reach above $80\%$ when $C> 2.0$ while for DLS mode when $C>2.0$, the accuracy level could arrive above $90\%$. Hence we come to a conclusion that a reference value for $C$ to achieve an acceptable prediction in the selected maze environment is 2.0. This will guide the later experiments in this paper.

Another interesting phenomenon in Fig.~\ref{fig:num_curves} is the accuracy for DLS mode has a faster convergence~(per coefficient $C$) comparing with the one for PLS mode even PLS mode has a perfect-sensing assumption. This implies that the LRMC model can have over-fitting issue if a perfect-sensing model is used and appropriate level of noise could relieve the problem and achieve a good accuracy with fewer observations. This characteristics is very important and useful since it implies the LRMC model is more suited to real-world scenarios. %, which is something we feel more interested in.

\begin{figure}%[h!]
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/pc.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/dc.png}
    \caption{}
  \end{subfigure}
  \caption{Prediction accuracy vs. coefficient $C$. Curves for (a)~PLS mode and (b)~DLS mode.}
  \label{fig:num_curves}
\end{figure}

==> old/5_experiments.tex <==
\section{EXPERIMENTS}
The goal of this paper is to demonstrate that a LRMC based map predictive coverage planning is useful and necessary for coverage scenarios in maze-like environments, particularly when the sensory raw measurements are noisy and sparse and the given energy is quite limited. We have shown that the maze-like environments fit well into the LRMC model. We want to understand in a further step how the model behaves in the context of coverage planning, instead of static discrete sampling as shown in Fig.~\ref{fig:demo}, and how our proposed method performs comparing with other alternative existing coverage planning techniques. We firstly describe our experimental setups and introduce all the methods involved in experiments and then conduct exhaustive analysis of coverage behaviors for different baseline methods and our proposed method with two sensing modes: PLS and DLS, respectively.

\begin{figure*}%[h!]
  \centering
  \begin{subfigure}[b]{0.19\linewidth}
    \includegraphics[width=\linewidth]{figs/map_truth.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.39\linewidth}
    \includegraphics[width=\linewidth]{figs/pls_1.0.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.39\linewidth}
    \includegraphics[width=\linewidth]{figs/dls_1.0.png}
    \caption{}
  \end{subfigure}
  \caption{\small (a)~Ground-truth maze map. (b)\textit{Left}: Real sensed map by TSP\_$1.0$ with PLS mode. The red points are random uniform sampled points while the yellow poly-lines are the shortest path found by TSP. The green blocks represent the missing parts in the map. \textit{Right}: Predicted map using the LRMC model. (c)\textit{Left}: Real sensed map by TSP\_$1.0$ with DLS mode. The color legends have the same meaning with the ones in (b). \textit{Right}: Predicted map using the LRMC model.}
  \label{fig:tsp_results}
\end{figure*}

\begin{table*}%[h]
\caption{Coverage performance comparison} %title of the table
\centering % centering table
\begin{tabular}{c rrrrrrrrr} % creating eight columns
\hline\hline %inserting double-line
% Properties&\multicolumn{7}{c}{Sum of Extracted Bits} \\ [0.5ex]
  & \vline & 20\% & 40\% & 50\% & 60\% & 80\% & 90\% & 100\% \\
\hline % inserts single-line
LM & \vline & 70 / 81 & 142 / 170 & 177 / 214 & 214 / 255 & 286 / 342 & 324 / - &  358 / -\\ [1ex]% Entering row contents
GR & \vline & 74 / 89 & 136 / 196 & 212 / 273 & 254 / 357 & 367 / - & 450 / - & - / -\\ [1ex]% [1ex] adds vertical space
FF & \vline & 85 / - & 166 / - & 205 / - & 257 / - & 365 / - & 418 / - & 500 / - \\ [1ex]
TSP\_0.75 & \vline & 34 / \textbf{29} & 70 / 53 & 86 / \textbf{68} & 105 / \textbf{86} & 155 / 131 & 176 / 146 & - / - \\ [1ex]
TSP\_1.0 & \vline & \textbf{32} / 33 & \textbf{60} / \textbf{68} & \textbf{61} / 86 & \textbf{71} / 105 & 143 / \textbf{141} & 167 / \textbf{157} & - / - \\ [1ex]
TSP\_1.25 & \vline & 34  / 32 & 70 / 67 & 84 / 83 & 114 / 101 & \textbf{137} / 156 & \textbf{165} / 180 & \textbf{241} / \textbf{235} \\
\hline % inserts single-line
\end{tabular}
\label{tb:coverage_comparison}
\end{table*}

\subsection{Experimental Setup}
We conduct our experiments based on the maze map as shown in Fig.~\ref{fig:tsp_results}-(a), which has a rank of 11. In this paper, we assume our vehicle for performing coverage mission is a point robot and no dynamics is considered. In Section.~\ref{sec:map_completion}, we have shown with a proper choice of $C$, the offline static map completion performance is outstanding and we also conclude there that a reference value for $C$ could be set to 2.0. However, in coverage planning, the observation entries are incrementally revealed since the robot needs to take time to traverse the area and only the places the robot has traversed could become observed entries in the matrix. To find a path for robot to traverse while following the random uniform observation pattern in the LRMC model, we first uniformly sample a set of points, then the sampled points are post-processed by an existing Traveling Salesman Problem~(TSP) solver to find a shortest path connecting all the sampled points. At first glance, the number of sampled points should be identical to the number of sampled observation blocks in the example in Section.~\ref{sec:map_completion}, where the samples number is defined as:
\begin{equation}
    \label{eq:sample_num}
    N^{'}_{s} = \left \lfloor \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N^{'}_{s}$ represents the samples number and $N$ is the number of observation entries within the robot local sensing range. Each sampled point will become a sampled block when the robot arrives at there. Nevertheless, in the coverage planning scenario, the robot can take observations in between a pair of connected sampled points and may introduce additional observations. This implies we may want to reduce the number of sampled points and we do this by introducing a scale factor $\epsilon$ to Eq.~(\ref{eq:sample_num}):
\begin{equation}
    \label{eq:new_sample_num}
    N_{s} = \left \lfloor \epsilon N^{'}_{s} \right \rfloor = \left \lfloor \epsilon \frac{C\cdot n^{1.2}r\log n}{N} \right \rfloor
\end{equation}
where $N_{s}$ is the new samples number and here we fix the value of $C$ as 2.0.

Once the points are sampled using Eq.~(\ref{eq:new_sample_num}), a shortest path will be formed using a TSP solver and thereafter our robot could start the coverage mission by following the path.

\begin{figure}%[h!]
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/pls_coverage.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/dls_coverage.png}
    \caption{}
  \end{subfigure}
  \caption{\small Coverage convergence of different methods for (a)~PLS mode and (b)~DLS mode.}
  \label{fig:coverage}
\end{figure}

\subsection{Introduction to Experimental Methods}
We now describe the baseline methods and our proposed method with different choices of parameters. The baseline methods we want to beat include: \textit{Lawn-Mower}~(LM) based coverage planning, \textit{Global Random Sampling}~(GRS) based coverage planning and \textit{Feature Frontier}~(FF) based coverage planning. 

\textit{LM}: A simple but widely used classical coverage planning method. Given the size of the mapping area, a path with carefully designed interval is computed such that the whole area could be swept incrementally by the robot.

\textit{GRS}: A global random sampling based method, in which at each action step, a set of points are randomly sampled in all unexplored areas and the closest one to the robot is selected as the local goal and a series of way-points are generated correspondingly. The robot only takes the first way-point for execution.

\textit{FF}: A feature frontier based method. The feature frontier here is defined as the intersections between the current explored areas boundary and the featured spaces. The featured spaces are defined as the places identified by an aerial robot from the air as having buildings. %This method tends to lead the robot to wander above the featured spaces and can easily stuck in local space if the local sensing is sparse and noisy due to the super sensitivity of the frontiers to noises.

Our proposed map predictive coverage planning method is based on TSP and hence we name our proposed method with different $\epsilon$ values as: $TSP\_\epsilon$, where the $\epsilon$ is the scale factor in Eq.~(\ref{eq:new_sample_num}) and will be replaced with some specific values in experiments.

\subsection{Coverage Quality Analysis}
We compare the coverage convergence performance~(per action step) of \textit{LM}, \textit{GRS}, \textit{FF} and $TSP\_\epsilon$, where $\epsilon \in \left \{ 0.25,~0.5,~0.75,~1.0,~1.25,~1.5,~1.75 \right \}$, for two local sensing modes, PLS and DLS on the same underlying maze map~(as shown in Fig.~\ref{fig:tsp_results}-(a)), respectively. The results are shown in Fig.~\ref{fig:coverage}. 

We first consider the coverage planning under PLS mode, where we assume the sensed local map for each action step is perfect, and the results are shown in Fig~\ref{fig:coverage}-(a). We can see that due to the functionality of prediction, our proposed TSP\_$\epsilon$ methods significantly outperform all the baseline methods in terms of coverage convergence, although TSP based method can reach different completeness level as the value of $\epsilon$ varies. Empirically a larger value of $\epsilon$ can lead to more sample points, a longer path~(and action step) from TSP, but as well as a better completeness~(i.e., TSP\_{1.5} and TSP\_(1.75)). A proper choice of $\epsilon$ value can give us a satisfactory trade-off between completeness and required action steps. For example, if we have enough energy supply and pursuit a well completed feature map, we should select a big value of $\epsilon$, such as 1.5 and 1.75. On the other hand, we can have a moderate magnitude $\epsilon$, like 0.75, 1.0 and 1.25 to achieve an acceptable coverage ratio~(i.e., 90\%), if we have limited energy or constrained allowed action steps. Even with extremely restricted number of action steps~(i.e., 110, 130, and 180), with a proper $\epsilon$, our TSP based method~(i.e., TSP\_{0.25}, TSP\_{0.5}, and TSP\_{0.75}) can still achieve $80\%(\pm 10\%)$ coverage. Although all baseline methods~(LM, GRS, and FF) can achieve good completeness, they require excessive action steps~(357, 603+, 500 for achieving 100\%~(or almost) coverage). If the maximum allowed number of actions is set as 130, none of the baseline methods could achieve a coverage that is more than 40\%.

In addition to the PLS mode, we also consider the coverage performance under DLS mode, which resembles the sensing quality in real hardware. The results are shown in Fig~\ref{fig:coverage}-(b). An exception for baseline methods is FF fails to perform the coverage mission because the detection of feature frontier is sensitive to the noises and heavily depends on map quality. In DLS mode, the obtained map contains many missing parts due to the sensor limits and noise. The robot is stuck in local area since there are always some feature frontiers are detected~(suppose the robot is within some places having featured spaces). Solving this problem may involve more robust frontier detection tricks, which are out of the scope of this paper. Other two baselines, LM and GRS, suffer from the bad sensing quality and have much slower convergence than themselves in PLS mode. On the contrary, our proposed TSP\_$\epsilon$ method is naturally robust to missing-ness and keep the same convergence performance as in PLS mode. We show the feature maps obtained at ending step of TSP\_{1.0} for PLS and DLS in Fig.~\ref{fig:tsp_results}-(b) and Fig.~\ref{fig:tsp_results}-(c), respectively.

We also list the required number of action steps of all baseline methods and our proposed TSP based method with three mild $\epsilon$ values for different levels of completeness in Table~\ref{tb:coverage_comparison}. The format for the entries in Table~\ref{tb:coverage_comparison} is $\#_{PLS} / \#_{DLS}$, which presents the required action numbers for PLS and DLS. It is clear to see that our TSP\_$\epsilon$ can achieve remarkable reduction for required action steps at all listed completeness quantiles.










==> old/6_conclusions.tex <==
\section{CONCLUSIONS}
In typical coverage planning tasks, with limited power supply, a single agent may have to stop the mission with a partially observed feature map. Given this background, this paper proposes a map predictive coverage planning method by leveraging the theory of \textit{Low-Rank Matrix Completion}~(LRMC). We model the urban terrain map as a maze-like map and carefully illustrate how maze-like environments fit well into the LRMC model. Then with intensive experiments, we demonstrate our proposed map predictive method significantly outperforms other coverage planning baseline methods in terms of feature map coverage convergence.
